Stochastic Bandits with Linear Constraints

We study a constrained contextual linear bandit setting, where the goal of the agent is to produce a sequence of policies, whose expected cumulative reward over the course of $T$ rounds is maximum, and each has an expected cost below a certain threshold $\tau$. We propose an upper-confidence bound algorithm for this problem, called optimistic pessimistic linear bandit (OPLB), and prove an $\widetilde{\mathcal{O}}(\frac{d\sqrt{T}}{\tau-c_0})$ bound on its $T$-round regret, where the denominator is the difference between the constraint threshold and the cost of a known feasible action. We further specialize our results to multi-armed bandits and propose a computationally efficient algorithm for this setting. We prove a regret bound of $\widetilde{\mathcal{O}}(\frac{\sqrt{KT}}{\tau - c_0})$ for this algorithm in $K$-armed bandits, which is a $\sqrt{K}$ improvement over the regret bound we obtain by simply casting multi-armed bandits as an instance of contextual linear bandits and using the regret bound of OPLB. We also prove a lower-bound for the problem studied in the paper and provide simulations to validate our theoretical results.

==> Constrained Bandits/abstract.tex <==
We study a constrained contextual linear bandit setting, where the goal of the agent is to produce a sequence of policies, whose expected cumulative reward over the course of $T$ rounds is maximum, and each has an expected cost below a certain threshold $\tau$. We propose an upper-confidence bound algorithm for this problem, called {\em optimistic pessimistic linear bandit} (OPLB), and prove an $\widetilde{\mathcal{O}}(\frac{d\sqrt{T}}{\tau-c_0})$ bound on its $T$-round regret, where the denominator is the difference between the constraint threshold and the cost of a known feasible action. We further specialize our results to multi-armed bandits and %show that there always exists a feasible optimal policy with at most $m+1$ arms being active, where $m$ is the number of linear constraints. We leverage this geometric property and 
propose a computationally efficient algorithm for this setting. We prove a regret bound of $\widetilde{\mathcal{O}}(\frac{\sqrt{KT}}{\tau - c_0})$ for this algorithm in $K$-armed bandits, which is a $\sqrt{K}$ improvement over the regret bound we obtain by simply casting multi-armed bandits as an instance of contextual linear bandits and using the regret bound of OPLB. We also prove a lower-bound for the problem studied in the paper and provide simulations to validate our theoretical results.  

%\mgh{The mention of lower-bound should be removed here, in case we do not have it.}

%We study a simple variation of the classical contextual bandit problem, where in addition to an emitted reward, there is another output which can be viewed as a cost for that arm. The goal is to find a reward maximizing policy while only using policies satisfying an expected cost constraint during all time steps during learning. We provide an upper confidence bound algorithm for the contextual bandit version of this problem and show a frequentist regret of order $\tilde{\mathcal{O}}(\frac{1}{\tau-c_0} d  T^{1/2} )$. Where $\tau-c_0$ is the difference between the cost $c_0$ of a known safe arm and the max cost threshold $\tau$. Additionally we further specialize our results to the $K$ multi-armed bandit case we show that there always exists an optimal solution which is either a single arm or a mixture solution on two arms. We leverage these geometric properties to propose an efficient algorithm with a frequentist regret of order $\tilde{\mathcal{O}}(\frac{1}{\tau - c_0} K^{1/2} T^{1/2})$ which we show is minimax optimal via a lower bound. We provide some simulations to further demonstrate the properties of our algorithms.


% Based on this, we provide a new bandit algorithm which converges to such a solution with regret guarantees.

% Additionally we further specialize our results to the multi armed bandits setting where we leverage geometric  

==> Constrained Bandits/defs.tex <==
% \newcommand{\BEAS}{\begin{eqnarray*}}
% \newcommand{\EEAS}{\end{eqnarray*}}
% \newcommand{\BEA}{\begin{eqnarray}}
% \newcommand{\EEA}{\end{eqnarray}}
% \newcommand{\BA}{\begin{align}}
% \newcommand{\EA}{\end{align}}
% \newcommand{\BAS}{\begin{align*}}
% \newcommand{\EAS}{\end{align*}}
% \newcommand{\BEQ}{\begin{equation}}
% \newcommand{\EEQ}{\end{equation}}
% \newcommand{\BIT}{\begin{itemize}}
% \newcommand{\EIT}{\end{itemize}}
% \newcommand{\BNUM}{\begin{enumerate}}
% \newcommand{\ENUM}{\end{enumerate}}
% \newcommand{\diag}{\mathop{\rm diag}}
% \newcommand{\Diag}{\mathop{\rm Diag}}
% \newcommand{\note}[1]{{\textbf{\color{red}#1}}}
% \newcommand{\E}{\mathbb{E}}
% \DeclareMathOperator\Var{Var}



% \newcommand{\R}{\mathbb{R}}
% \DeclareMathOperator\tr{Tr}
% \newcommand{\ba}{B^{-1}A}
% \newcommand{\eps}{\varepsilon}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{corollary}{Corollary}[theorem]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newcommand{\mysec}[1]{Section~\ref{sec:#1}}
% \newcommand{\eq}[1]{Eq.~(\ref{eq:#1})}
% \newcommand{\myfig}[1]{Figure~\ref{fig:#1}}
% \newcommand{\myalgo}[1]{Algorithm~\ref{algo:#1}}
% \newcommand{\myapp}[1]{Appendix~\ref{sec:#1}}





\usepackage{url}
\usepackage{graphicx}
\usepackage[font=scriptsize]{caption}
\usepackage{amsmath}
\def\UrlFont{\rmfamily}
\usepackage{amsfonts}
%\usepackage{subcaption}
\usepackage{graphicx} % omit 'demo' for real document
% \usepackage[colorlinks,linkcolor=blue,citecolor=blue,urlcolor=blue]{hyperref}
%\usepackage[round,sort]{natbib}
\usepackage{natbib}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\usepackage{xcolor}
%\usepackage{algorithm}
%\usepackage{algorithm,algorithmic}
%\usepackage{algorithmic}
%\usepackage[algo2e]{algorithm2e}
\usepackage{tabularx} % also loads 'array' package
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{multirow}
\usepackage{bbm}
\usepackage{wrapfig}


\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newcounter{assump}
\newtheorem{assumption}[assump]{Assumption}



\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\note}[1]{\red{#1}}
\newcommand{\vct}[1]{#1}
\newcommand{\mtx}[1]{#1}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\unif}{Unif}
\DeclareMathOperator*{\dom}{dom}

\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator*{\cl}{cl}
\DeclareMathOperator*{\bd}{bd}
\DeclareMathOperator*{\Span}{span}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\sol}{SOL}
\DeclareMathOperator*{\dsol}{DSOL}
\DeclareMathOperator*{\vi}{VI}
\DeclareMathOperator*{\fp}{FP}
\DeclareMathOperator*{\dvi}{DVI}
\DeclareMathOperator*{\qvi}{QVI}
\DeclareMathOperator*{\cp}{CP}
\DeclareMathOperator*{\interior}{int}
\DeclareMathOperator*{\ncp}{NCP}
\DeclareMathOperator*{\mcp}{MCP}
\DeclareMathOperator*{\lcp}{LCP}
% \DeclareMathOperator*{\st}{s.t.}
\newcommand{\Tr}{\mathrm{Tr}}
\usepackage{enumitem}
\usepackage{wrapfig}

\newcommand{\st}{\text{ s.t. }}
\newcommand{\beq}{\begin{equation}}
\newcommand{\typicalset}{A^n_\epsilon}
\newcommand{\iid}{\stackrel{\text{iid}}{\sim}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqs}{\begin{equation*}}
\newcommand{\eeqs}{\end{equation*}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\nystrom}{Nystr\"{o}m}
\newcommand{\nlim}{\lim_{n \rightarrow \infty}}

\newcommand{\relint}{\text{relint}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\K}{\mathcal{K}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\kl}{\text{KL}}
\newcommand{\define}{\stackrel{\text{def.}}{=}}
\newcommand{\regret}{\text{Regret}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Tau}{\mathcal{T}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\z}{\mathcal{Z}}
\newcommand{\HS}{\mathcal{H}}
\newcommand{\ind}{\mathbf{1}}
% \newcommand{\1}{\mathbbm{1}}
\newcommand{\1}{\mathbf{1}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
% \renewcommand{\{}{\left\{}
% \renewcommand{\}}{\left\}}
\newcommand{\ip}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\Normal}{\mathcal{N}}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\abs}[1]{\ensuremath{| #1 |}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}

\newcommand{\g}{\mathbf{g}}
\newcommand{\q}{\mathbf{q}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\T}{\mathsf{T}}
\renewcommand{\Pr}{\mathbb{P}}
\renewcommand{\P}{\mathcal{P}}
\renewcommand{\T}{\mathcal{T}}

%\usepackage[margin=1.25in]{geometry}

%\newcommand{\aldo}[1]{\textcolor{red}{\it {\bf Aldo:} {#1}}}
%\newcommand{\mgh}[1]{\textcolor{blue}{\it {\bf MGH:} {#1}}}

% \newenvironment{oneshot}[1]{\@begintheorem{#1}{\unskip}}{\@endtheorem}



\usepackage[framemethod=TikZ]{mdframed}
\usepackage{amsthm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Theorem
\newcounter{theo}[section] \setcounter{theo}{0}
\renewcommand{\thetheo}{\arabic{section}.\arabic{theo}}
\newenvironment{theo}[2][]{%
\refstepcounter{theo}%
\ifstrempty{#1}%
{\mdfsetup{%
frametitle={%
\tikz[baseline=(current bounding box.east),outer sep=0pt]
\node[anchor=east,rectangle,fill=blue!20]
{\strut Theorem~\thetheo};}}
}%
{\mdfsetup{%
frametitle={%
\tikz[baseline=(current bounding box.east),outer sep=0pt]
\node[anchor=east,rectangle,fill=blue!20]
{\strut Theorem~\thetheo:~#1};}}%
}%
\mdfsetup{innertopmargin=5pt,linecolor=blue!20,%
linewidth=2pt,topline=true,%
frametitleaboveskip=\dimexpr-\ht\strutbox\relax
}
\begin{mdframed}[]\relax%
\label{#2}}{\end{mdframed}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Lemma
\newcounter{lem}[section] \setcounter{lem}{0}
\renewcommand{\thelem}{\arabic{section}.\arabic{lem}}
\newenvironment{lem}[2][]{%
\refstepcounter{lem}%
\ifstrempty{#1}%
{\mdfsetup{%
frametitle={%
\tikz[baseline=(current bounding box.east),outer sep=0pt]
\node[anchor=east,rectangle,fill=green!20]
{\strut Lemma~\thelem};}}
}%
{\mdfsetup{%
frametitle={%
\tikz[baseline=(current bounding box.east),outer sep=0pt]
\node[anchor=east,rectangle,fill=green!20]
{\strut Lemma~\thelem:~#1};}}%
}%
\mdfsetup{innertopmargin=10pt,linecolor=green!20,%
linewidth=2pt,topline=true,%
frametitleaboveskip=\dimexpr-\ht\strutbox\relax
}
\begin{mdframed}[]\relax%
\label{#2}}{\end{mdframed}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Proof
\newcounter{prf}[section]\setcounter{prf}{0}
\renewcommand{\theprf}{\arabic{section}.\arabic{prf}}
\newenvironment{prf}[2][]{%
\refstepcounter{prf}%
\ifstrempty{#1}%
{\mdfsetup{%
frametitle={%
\tikz[baseline=(current bounding box.east),outer sep=0pt]
\node[anchor=east,rectangle,fill=red!20]
{\strut Proof~\theprf};}}
}%
{\mdfsetup{%
frametitle={%
\tikz[baseline=(current bounding box.east),outer sep=0pt]
\node[anchor=east,rectangle,fill=red!20]
{\strut Proof~\theprf:~#1};}}%
}%
\mdfsetup{innertopmargin=10pt,linecolor=red!20,%
linewidth=2pt,topline=true,%
frametitleaboveskip=\dimexpr-\ht\strutbox\relax
}
\begin{mdframed}[]\relax%
\label{#2}}{\qed\end{mdframed}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Corollary
\newcounter{cor}[section]\setcounter{cor}{0}
\renewcommand{\thecor}{\arabic{section}.\arabic{cor}}
\newenvironment{cor}[2][]{%
\refstepcounter{cor}%
\ifstrempty{#1}%
{\mdfsetup{%
frametitle={%
\tikz[baseline=(current bounding box.east),outer sep=0pt]
\node[anchor=east,rectangle,fill=orange!20]
{\strut Corollary~\thecor};}}
}%
{\mdfsetup{%
frametitle={%
\tikz[baseline=(current bounding box.east),outer sep=0pt]
\node[anchor=east,rectangle,fill=yellow!20]
{\strut Corollary~\thecor:~#1};}}%
}%
\mdfsetup{innertopmargin=10pt,linecolor=orange!20,%
linewidth=2pt,topline=true,%
frametitleaboveskip=\dimexpr-\ht\strutbox\relax
}
\begin{mdframed}[]\relax%
\label{#2}}{\qed\end{mdframed}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Proposition
\newcounter{prop}[section] \setcounter{prop}{0}
\renewcommand{\thelem}{\arabic{section}.\arabic{prop}}
\newenvironment{prop}[2][]{%
	\refstepcounter{prop}%
	\ifstrempty{#1}%
	{\mdfsetup{%
			frametitle={%
				\tikz[baseline=(current bounding box.east),outer sep=0pt]
				\node[anchor=east,rectangle,fill=purple!20]
				{\strut Proposition~\thelem};}}
	}%
	{\mdfsetup{%
			frametitle={%
				\tikz[baseline=(current bounding box.east),outer sep=0pt]
				\node[anchor=east,rectangle,fill=purple!20]
				{\strut Proposition~\thelem:~#1};}}%
	}%
	\mdfsetup{innertopmargin=10pt,linecolor=purple!20,%
		linewidth=2pt,topline=true,%
		frametitleaboveskip=\dimexpr-\ht\strutbox\relax
	}
	\begin{mdframed}[]\relax%
		\label{#2}}{\end{mdframed}}


\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}


==> Constrained Bandits/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
\vspace{-0.1in}

% \begin{wrapfigure}{r}{0.72\textwidth}
%         \vspace{-5mm}
%         \begin{minipage}{0.72\textwidth}
%         \centering\subfigure{\includegraphics[width=0.3\linewidth]{figs/constrained_regrets_tau_1.png}} 
%         \centering\subfigure{\includegraphics[width=0.3\linewidth]{figs/cost_evolution_tau_1.png}} 
%         \centering\subfigure{\includegraphics[width=0.3\linewidth]{figs/rewards_evolution_tau_1.png}} 
%         \end{minipage}
%         \vspace{-5mm}
%         \caption{\small{ Threshold $\tau = 1$.}}
%         \vspace{-3mm}
%         \label{fig:constrained_bandits1}
%         %\vspace{-5mm}
%         \begin{minipage}{0.72\textwidth}
%         \centering\subfigure{\includegraphics[width=0.3\linewidth]{figs/constrained_regrets_tau_05.png}} 
%         \centering\subfigure{\includegraphics[width=0.3\linewidth]{figs/cost_evolution_tau_05.png}} 
%         \centering\subfigure{\includegraphics[width=0.3\linewidth]{figs/rewards_evolution_tau_05.png}} 
%         \end{minipage}
%         \vspace{-5mm}
%         \caption{\small{ Threshold $\tau = 0.5$. }}
%         \vspace{-3mm}
%         \label{fig:constrained_bandits1}
% %        \vspace{-5mm}
%         \begin{minipage}{0.72\textwidth}
%         \centering\subfigure{\includegraphics[width=0.3\linewidth]{figs/constrained_regrets_tau_02.png}} 
%         \centering\subfigure{\includegraphics[width=0.3\linewidth]{figs/cost_evolution_tau_02.png}} 
%         \centering\subfigure{\includegraphics[width=0.3\linewidth]{figs/rewards_evolution_tau_02.png}} 
%         \end{minipage}
%         \vspace{-5mm}
%         \caption{\small{Threshold $\tau = 0.2$.}}
%         %\vspace{1mm}
%         \label{fig:constrained_bandits1}
% \begin{center}
%     \begin{minipage}{0.65\textwidth}
% \begin{center}   \small{ \textbf{OPB.} Bernoulli arms. $\bar{r} = (.1, .2, .4, .7)$, $\bar{c}=(0, .4, .5, .2)$, $c_0 = 0$.} \end{center}
%     \end{minipage}
%     \end{center}
% \end{wrapfigure}

We run a set of experiments to show the behavior of OPB and validate our theoretical results. We consider a $K=4$-armed bandits in which the reward and cost distributions of the arms are Bernoulli with means $\bar r=(.1,.2,.4,.7)$ and $\bar c =(0,.4,.5,.2)$. So, the cost of the safe arm is $\bar c_1=0$. In Figures~\ref{fig:constrained_bandits1} to~\ref{fig:constrained_bandits3}, we gradually reduce the constraint threshold $\tau$, and as a result the complexity of the problem $\tau - \bar{c}_1$, and show the regret {\em (left)} and the cost {\em (middle)} and reward {\em (right)} evolution of OPB. All the results are averaged over $10$ runs and the shade is the $\pm .5$ standard deviation around the regret. 

Our results show that the regret of OPB grows as we reduce $\tau$ {\em (left)}. They also indicate that the algorithm is successful in satisfying the constraint {\em (middle)} and reaching the optimal reward/performance {\em (right)}. In Figure~\ref{fig:constrained_bandits3}, the reason that the cost evolution of OPB is the same as that of the optimal policy {\em (middle)} is that in this case, the cost of the best arm (arm $4$) is equal to the constraint threshold $\tau=.2$. 

%In this section we should some simple plots capturing the behavior of OPB in the multi armed bandit setting. It can be appreciated that in the same bandit instance, a decreasing cost threshold has an impact on the constrained regret of the algorithm. Each experiment was run over 10 random seeds, and $\pm .5$ standard deviation curves are shaded around the regret, expected costs and expected rewards signals.  

\begin{wrapfigure}{r}{0.625\textwidth}
        %\vspace{-5mm}
        \vspace{-0.3in}    
        \begin{minipage}{0.625\textwidth}%\hspace{-0.1in}
        \centering\subfigure{\includegraphics[width=0.325\linewidth]{figs/constrained_regrets_tau_1.png}} 
        \centering\subfigure{\includegraphics[width=0.325\linewidth]{figs/cost_evolution_tau_1.png}} 
        \centering\subfigure{\includegraphics[width=0.325\linewidth]{figs/rewards_evolution_tau_1.png}} 
        \end{minipage}
        \vspace{-4mm}
        \caption{{Constraint Threshold $\;\tau = 1$.}}
        \vspace{-2mm}
        \label{fig:constrained_bandits1}
        %\vspace{-5mm}
        \begin{minipage}{0.625\textwidth}%\hspace{-0.1in}
        \centering\subfigure{\includegraphics[width=0.325\linewidth]{figs/constrained_regrets_tau_05.png}} 
        \centering\subfigure{\includegraphics[width=0.325\linewidth]{figs/cost_evolution_tau_05.png}} 
        \centering\subfigure{\includegraphics[width=0.325\linewidth]{figs/rewards_evolution_tau_05.png}} 
        \end{minipage}
        \vspace{-4mm}
        \caption{{Constraint Threshold $\;\tau = 0.5$.}}
        \vspace{-2mm}
        \label{fig:constrained_bandits2}
%        \vspace{-5mm}
        \begin{minipage}{0.625\textwidth}%\hspace{-0.1in}
        \centering\subfigure{\includegraphics[width=0.325\linewidth]{figs/constrained_regrets_tau_02.png}} 
        \centering\subfigure{\includegraphics[width=0.325\linewidth]{figs/cost_evolution_tau_02.png}} 
        \centering\subfigure{\includegraphics[width=0.325\linewidth]{figs/rewards_evolution_tau_02.png}} 
        \end{minipage}
        \vspace{-4mm}
        \caption{{Constraint Threshold $\;\tau = 0.2$.}}
        %\vspace{1mm}
        \label{fig:constrained_bandits3}
\begin{center}
\begin{minipage}{0.625\textwidth}
\begin{center}   \small{ \textbf{OPB.} Bernoulli arms. $\bar{r} = (.1, .2, .4, .7)$, $\bar{c}=(0, .4, .5, .2)$, $\bar{c}_1 = 0$.} \end{center}
    \end{minipage}
    \end{center}
\vspace{-0.225in}    
\end{wrapfigure}


% \begin{figure}[h]
% \includegraphics[width=.3\textwidth]{figs/constrained_regrets_tau_1.png} 
% \includegraphics[width=.3\textwidth]{figs/cost_evolution_tau_1.png}
% \includegraphics[width=.3\textwidth]{figs/rewards_evolution_tau_1.png}
% \caption{Constrained Multi Armed Bandits. Bernoulli reward means $.1, .2, .4, .7$ cost means $0, .4, .5, .2$. Threshold $\tau = 1$. Known arm with cost $0$. }
%     \label{fig:constrained_bandits1}
% \includegraphics[width=.3\textwidth]{figs/constrained_regrets_tau_05.png} 
% \includegraphics[width=.3\textwidth]{figs/cost_evolution_tau_05.png}
% \includegraphics[width=.3\textwidth]{figs/rewards_evolution_tau_05.png}
% \caption{Constrained Multi Armed Bandits. Bernoulli reward means $.1, .2, .4, .7$ cost means $0, .4, .5, .2$. Threshold $\tau = .5$. Known arm with cost $0$. }
%     \label{fig:constrained_bandits2}
% \includegraphics[width=.3\textwidth]{figs/constrained_regrets_tau_02.png} 
% \includegraphics[width=.3\textwidth]{figs/cost_evolution_tau_02.png}
% \includegraphics[width=.3\textwidth]{figs/rewards_evolution_tau_02.png}
% \caption{Constrained Multi Armed Bandits. Bernoulli reward means $.1, .2, .4, .7$ cost means $0, .4, .5, .2$. Threshold $\tau = .2$. Known arm with cost $0$. }
%     \label{fig:constrained_bandits3}
% \end{figure}





==> Constrained Bandits/introduction.tex <==
\section{Introduction}
\label{sec:intro}

A {\em multi-armed bandit} (MAB)~\citep{lai85asymptotically,auer02finitetime,lattimore2018bandit} is an online learning problem in which the agent acts by pulling arms. After an arm is pulled, the agent receives its {\em stochastic reward}. The goal of the agent is to maximize its expected cumulative reward without knowledge of the arms' distributions. To achieve this goal, the agent has to balance its {\em exploration} and {\em exploitation}: to decide when to {\em explore} and learn about the arms, and when to {\em exploit} and pull the arm with the highest estimated reward thus far. A \emph{stochastic linear bandit}~\citep{dani08stochastic,rusmevichientong10linearly,abbasi2011improved} is a generalization of MAB to the setting where each of (possibly) infinitely many arms is associated with a feature vector. The mean reward of an arm is the dot product of its feature vector and an unknown parameter vector, which is shared by all the arms. This formulation contains time-varying action (arm) sets and feature vectors, and thus, includes the {\em linear contextual bandit} setting. These models capture many practical applications spanning clinical trials~\citep{Villar15MA}, recommendation systems~\citep{Li10CB,balakrishnan2018using}, wireless networks~\citep{maghsudi2016multi}, sensors~\citep{washburn2008application}, and strategy games \citep{ontanon2013combinatorial}. 
The most popular exploration strategies in stochastic bandits are {\em optimism in the face of uncertainty} (OFU)~\citep{auer02finitetime} and {\em Thompson sampling} (TS)~\citep{thompson33likelihood,agrawal13further,russo18tutorial} that are relatively well understood in both multi-armed and linear bandits~\citep{dani08stochastic,abbasi2011improved,agrawal13thompson,lattimore2018bandit}.

In many practical problems, the agent requires to satisfy certain operational constraints while maximizing its cumulative reward. Depending on the form of the constraints, several {\em constrained stochastic bandit} settings have been formulated and analyzed. One such setting is what is known as {\em knapsack bandits}. In this setting, pulling each arm, in addition to producing a reward signal, results in a random consumption of a global budget, and the goal is to maximize the cumulative reward before the budget is fully consumed (e.g.,~\citealt{badanidiyuru2013bandits,badanidiyuru2014resourceful,agrawal2014bandits,wu2015algorithms,agrawal2016linear}). Another such setting is referred to as {\em conservative bandits}. In this setting, there is a baseline arm or policy, and the agent, in addition to maximizing its cumulative reward, should ensure that at each round, the difference between its cumulative reward and that of the baseline remains below a predefined fraction of the baseline cumulative reward~\citep{wu2016conservative,kazerouni2017conservative,Garcelon20IA}. In these two settings, the constraint applies to a cumulative quantity (budget consumption or reward) over the entire run of the algorithm. Thus, the set of feasible actions at each round is a function of the history of the algorithm. 

Another constrained bandit setting is where each arm is associated with two (unknown) distributions, generating reward and cost signals. The goal is to maximize the cumulative reward, while making sure that with high probability, the expected cost of the arm pulled at each round is below a certain threshold. Here the constraint is stage-wise, and unlike the last two settings, is independent of the history.~\citet{amani2019linear} and~\citet{Moradipari19SL} have recently studied this setting for linear bandits and derived and analyzed explore-exploit~\citep{amani2019linear} and Thompson sampling~\citep{Moradipari19SL} algorithms for it. 

This setting is the closest to the one we study in this paper. In our setting, we also assume two distributions for each arm, one for reward and for cost. At each round the agent constructs a policy according to which it takes its action. The goal of the agent is to produce a sequence of policies with maximum expected cumulative reward, while making sure that the expected cost of the constructed policy (not the pulled arm) at each round is below a certain threshold. This is a linear constraint and can be easily extended to more constraints by having more cost distributions associated to each arm, one per each constraint. Compared to the previous setting, our constraint is more relaxed (from high-probability to expectation), and as a result, it would be possible for us to obtain a solution with larger expected cumulative reward. We will have a detailed discussion on the relationship between these two settings and the similarities and differences of our results with those reported in~\citet{amani2019linear} and~\citet{Moradipari19SL} in Section~\ref{sec:related-work}.

In this paper, we study the above setting for contextual linear bandits. After defining the setting in Section~\ref{sec:setting}, we propose an upper-confidence bound (UCB) algorithm for it, called {\em optimistic pessimistic linear bandit} (OPLB), in Section~\ref{sec:algo}. We prove an $\widetilde{\mathcal{O}}(\frac{d\sqrt{T}}{\tau-c_0})$ bound on the $T$-round regret of OPLB in Section~\ref{section::lin_opt_pess_analysis}, where $d$ is the action dimension and $\tau-c_0$ is the difference between the constraint threshold and the cost of a known feasible action. The action set considered in our contextual linear bandit setting is general enough to include MAB. However, in Section~\ref{sec:constrained-MAB}, we further specialize our results to MAB and propose a computationally efficient algorithm for this setting, called {\em optimistic pessimistic bandit} (OPB). We show that in the MAB case, there always exists a feasible optimal policy with probability mass on at most $m+1$ arms, where $m$ is the number of linear constraints. This property plays an important role in the computational efficiency of OPB. We prove a regret bound of $\widetilde{\mathcal{O}}(\frac{\sqrt{KT}}{\tau - c_0})$ for OPB in $K$-armed bandits, which is a $\sqrt{K}$ improvement over the regret bound we obtain by simply casting MAB as an instance of contextual linear bandit and using the regret bound of OPLB. We also prove a lower-bound for the problem studied in the paper and provide simulations to validate our theoretical results.

%\mgh{The mention of lower-bound should be removed here, in case we do not have it.}

% Multi-armed bandits (MABs) \cite{audibert2010best} have had a considerable impact on machine learning and have been studied extensively. In this paper, we introduce a simple variation, called {\it constrained bandits}, where in addition to an emitted reward, there is another output which can be viewed as a cost or bounty for that arm. The goal is then to find an optimal policy which satisfies a constraint on the cost or bounty across time.

% Perhaps the simplest case of the constrained bandits is where the reward itself is taken as the other output and the constraint is that the average reward must exceed a certain threshold at any given time. This is useful in applications where one wants to maximize revenues but also strictly ensure that at any given point in time, the total revenue always exceeds a certain amount (i.e. the expenses) to avoid being in a net negative state even if a more profitable (but has a chance of going into a net negative state) solution exists. This simple case of constrained bandits can be useful in similar problems: for example in designing real-time interactive systems where the designer benefits from participants, but must ensure at any point to not give an overall negative experience to the participants to avoid losing users.

% We next consider the more general case of constrained bandits where the other output is not necessarily the same as the reward.
% One example is the problem of learning decision thresholds across time. In many practical binary classification problems such as predicting when to trigger on an event or whether to show an advertisement, learning the classifier and determining the optimal decision threshold are done separately. It may be important that the system not only optimizes for accuracy, but also ensures constraints that the learner has as any given time. For instance, when showing ads, a given ads campaign might only have a certain budget and thus the problem is not only to choose the ads with highest probability of engagement, but also to have the constraint that the total cost of the ads shown is aligned with the campaign's spend schedule across time.

% Lastly, an important application of the constrained bandits is ML fairness. One specific instance is the problem of granting loans on a rolling basis. While the goal may be to grant loans to those with the highest chance of repayment, there may be an additional constraint that a minority group's overall proportion of approval must exceed a certain cutoff (i.e. enforced by regulators) at {\it any given time}. It is significant to note that the bulk of the group-based fairness research has been focused on the passive setting-- that is, the learner receives all of the datapoints at the beginning and can make decisions knowing the data distribution in advance. However, it is more realistic in many settings that these decisions need to be made with limited turn-around time. Thus, while the focus of the paper is not on fairness, this setting may be of interest to the ML fairness community.

% Despite the potential wide significance of constrained bandits, there has been little work done in online learning with constraints, which we will discuss in the related works section. Our contributions include (1) introducing the formulation for the constrained bandits problem; (2) providing a striking result that says there always exists an optimal solution which is either a single arm or a mixture solution supported on two arms. (3) giving a new bandit procedure based on this observation which converges with regret guarantees to such a solution.




==> Constrained Bandits/linear_bandits.tex <==
\section{Problem Formulation}
\label{sec:setting}

We adopt the following notation. The set $\{1,\ldots,T\}$ is denoted by $[T]$. We represent the set of distributions with support over a compact set $\mathcal S$ by $\Delta_{\mathcal S}$. We denote by $\langle x,y \rangle:=x^\top y\in\mathbb R$, the inner product of two vectors $x,y\in\mathbb R^d$, and by $\|x\|:=\sqrt{x^\top x}$, the $\ell_2$-norm of vector $x$. 

The setting we study in this paper is {\em contextual linear bandit} with {\em linear constraints}. In each round $t$, the agent is given an decision set $\mathcal A_t\subset{\mathbb R}^d$ from which it has to choose an action $x_t$. Upon taking action $x_t\in\mathcal A$, it observes a pair $(r_t,c_t)$, where $r_t=\langle x_t,\theta_*\rangle + \xi^r_t$ and $c_t=\langle x_t,\mu_*\rangle + \xi^c_t$ are the reward and cost signals, respectively. In the reward and cost definitions, $\theta_*\in{\mathbb R}^d$ and $\mu_*\in{\mathbb R}^d$ are the unknown {\em reward} and {\em cost parameters}, and $\xi^r_t$ and $\xi^c_t$ are reward and cost noise, satisfying conditions that will be specified soon. The agent selects its action $x_t\in\mathcal A_t$ in each round $t$ according to its policy $\pi_t\in\Delta_{\mathcal A_t}$ at that round, i.e.,~$x_t\sim\pi_t$. 

The goal of the agent is to produce a sequence of policies $\{\pi_t\}_{t=1}^T$ with maximum {\em expected cumulative reward} over the course of $T$ rounds, while satisfying the {\bf\em linear constraint} 
%
\begin{equation}
\label{eq:constraint}
\mathbb E_{x\sim\pi_t}[\langle x,\mu_* \rangle]\leq \tau,\quad\forall t\in[T], \qquad (\tau\geq 0 \;\; \text{is referred to as the \em constraint threshold}). 
\end{equation}
%
Thus, the policy $\pi_t$ selected by the agent in each round $t\in [T]$ should belong to the set of {\em feasible policies} over the action set $\mathcal A_t$, i.e.,~$\Pi_t=\{\pi\in\Delta_{\mathcal A_t}:\mathbb E_{x\sim\pi}[\langle x,\mu_* \rangle]\leq \tau\}$. Maximizing the expected cumulative reward in $T$ rounds is equivalent to minimizing the $T$-round {\em constrained pseudo-regret},\footnote{In the rest of the paper, we simply refer to the $T$-round constrained pseudo-regret $\mathcal R_\Pi(T)$ as $T$-round regret.}
%
% \vspace{-0.15in}
% \begin{small}
\begin{equation}
\label{eq:regret}
\mathcal R_\Pi(T) = \sum_{t=1}^T \mathbb E_{x\sim\pi_t^*}[\langle x,\theta_* \rangle] - E_{x\sim\pi_t}[\langle x,\theta_* \rangle], 
\end{equation}
% \end{small}
% \vspace{-0.15in}
%
where $\pi_t,\pi^*_t\in\Pi_t\;\forall t\in[T]$ and $\pi^*_t$ is the {\em optimal feasible} policy at round $t$, i.e.,~$\pi^*_t\in\max_{\pi\in\Pi_t}\mathbb E_{x\sim\pi}[\langle x,\theta_* \rangle]$. The terms $\mathbb E_{x\sim\pi}[\langle x,\theta_* \rangle]$ and $\mathbb E_{x\sim\pi}[\langle x,\mu_* \rangle]$ in~\eqref{eq:constraint} and~\eqref{eq:regret} are the expected reward and cost of policy $\pi$, respectively. Thus, a feasible policy is the one whose expected cost is below the constraint threshold $\tau$, and the optimal feasible policy is a feasible policy with maximum expected reward. We use the shorthand notations $x_\pi := \mathbb{E}_{x \sim \pi}[x]$, $r_\pi:=\mathbb E_{x\sim\pi}[\langle x,\theta_* \rangle]$ and $c_\pi:=\mathbb E_{x\sim\pi}[\langle x,\mu_* \rangle]$ for the expected action, reward and cost of a policy $\pi$. With these shorthand notations, we may write the $T$-round pseudo-regret as $\mathcal R_\Pi(T)=\sum_{t=1}^T r_{\pi^*_t} - r_{\pi_t}$.

We make the following assumptions for our setting. The first four assumptions are standard in linear bandits. The fifth one is necessary to guarantee constraint satisfaction ({\em safety}). 

\begin{assumption}
\label{ass:noise-sub-gaussian}
For all $t\in[T]$, the reward and cost noise random variables $\xi_t^r$ and $\xi_t^c$ are conditionally $R$-sub-Gaussian, i.e.,
%
% \vspace{-0.15in}
% \begin{small}
\begin{align*}
&\mathbb{E}[\xi_t^r \mid \mathcal{F}_{t-1}] = 0, \qquad \mathbb{E}[\exp(\alpha \xi_t^r) \mid \mathcal{F}_{t-1}] \leq \exp(\alpha^2 R^2/2),\;\;\;\forall \alpha\in\mathbb R, \\
&\mathbb{E}[\xi_t^c \mid \mathcal{F}_{t-1}] = 0, \qquad \mathbb{E}[\exp(\alpha \xi_t^c) \mid \mathcal{F}_{t-1}] \leq \exp(\alpha^2 R^2/2),\;\;\;\forall \alpha\in\mathbb R,
\end{align*}
% \end{small}
% \vspace{-0.15in}
%
where $\mathcal F_t$ is the filtration that includes all the events $(x_{1:t+1},\xi^r_{1:t},\xi^c_{1:t})$ until the end of round $t$.
\end{assumption}
%
\begin{assumption}
\label{ass:bounded-reward-cost-param}
There is a known constant $S > 0$, such that $\| \theta_*\| \leq S$ and $\| \mu_*\| \leq S$.\footnote{The choice of the same upper-bounds for $\theta_*$ and $\mu_*$ is just for simplicity.}
\end{assumption}
%
\begin{assumption}
\label{ass:bounded-action}
The $\ell_2$-norm of all actions is bounded, i.e.,~$\max_{t\in[T]}\max_{x \in \mathcal{A}_t}\| x \|  \leq L$. 
\end{assumption}
%
\begin{assumption}
\label{ass:bounded-mean-reward-cost}
For all $t\in[T]$ and $x \in \mathcal{A}_t$, the mean rewards and costs are bounded, i.e.,~$\langle x, \theta_* \rangle \in [0,1]$ and $\langle x, \mu_* \rangle \in [0,1]$.
\end{assumption}
%
\begin{assumption}
\label{ass:safe-action}
There is a known safe action $x_0\in\mathcal A_t,\;\forall t\in[T]$ with known %\footnote{If $c_0$ is unknown, it can be estimated by playing the safe arm $x_0$ at the cost of only $\sqrt{T}$ regret.} 
cost $c_0$, i.e.,~$\langle x_0, \mu_* \rangle = c_0 < \tau$. We will show how the assumption of knowing $c_0$ can be relaxed later in the paper.
\end{assumption}
%
{\bf Notation:} We conclude this section with introducing another set of notations that will be used in the rest of the paper. We define the normalized safe action as $e_0:=x_0/\|x_0\|$ and the span of the safe action as $\mathcal{V}_o := \mathrm{span}(x_0) =\{\eta x_0 : \eta\in\mathbb R\}$. We denote by $\mathcal{V}_o^{\perp}$, the orthogonal complement of $\mathcal{V}_o$, i.e.,~$\mathcal{V}_o^{\perp}=\{x\in\mathbb R^d : \langle x,y\rangle=0,\;\forall y\in\mathcal{V}_o\}$.\footnote{In the case of $x_0 = \mathbf{0}\in\mathbb R^d$, we define $\mathcal{V}_o$ as the empty subspace and $\mathcal{V}_o^\perp$ as the whole $\mathbb{R}^d$.} We define the projection of a vector $x\in\mathbb R^d$ into the sub-space $\mathcal{V}_o$, as $x^o:=\langle x,e_0\rangle e_0$, and into the sub-space $\mathcal{V}_o^{\perp}$, as $x^{o,\perp} := x - x^o$. We also define the projection of a policy $\pi$ into $\mathcal{V}_o$ and $\mathcal{V}_o^{\perp}$, as $x_{\pi}^o := \mathbb{E}_{x \sim \pi}[x^o]$ and $x_{\pi}^{o, \perp} := \mathbb{E}_{x \sim \pi}[x^{o, \perp}]$. %Finally, we decompose the cost parameter $\mu_*$ along the sub-spaces $\mathcal{V}_o$ and $\mathcal{V}_o^{\perp}$ as $\mu_*^o := \langle \mu_*,e_0 \rangle e_0=  \frac{c_0}{\|x_0\|}e_0$ and $\mu_*^{o,\perp} = \mu_* - \mu_*^o$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Optimistic-Pessimistic Linear Bandit Algorithm}
\label{sec:algo}

In this section, we propose an algorithm, called {\em optimistic-pessimistic linear bandit} (OPLB), whose pseudo-code is shown in Algorithm~\ref{alg:optimistic-pessimistic-LB}. Our OPLB algorithm balances a pessimistic assessment of the set of available policies, while acting optimistically within this set. Our principal innovation is the use of confidence intervals with asymmetric radii, proportional to $\alpha_r$ and $\alpha_c$, for the reward and cost signals. This will prove crucial in the regret analysis of the algorithm. 
 
{\centering
\begin{minipage}{.9\linewidth}
    \begin{algorithm}[H]
    \textbf{Input:} \begin{small}Horizon $T$, Confidence Parameter $\delta$, Regularization Parameter $\lambda$, Constants $\alpha_r, \alpha_c \geq 1$\end{small} \\
    \For{$t=1,\ldots,T$}{
    1. Compute RLS estimates $\;\widehat{\theta}_t\;$ and $\;\widehat{\mu}_t^{o,\perp}$ \hfill {\em (see Eqs.~\ref{eq:param-est} to~\ref{eq:proj-est})} \\
    2. Construct sets $\;\mathcal{C}_t^r(\alpha_r)\;$ and $\;\mathcal{C}_t^c(\alpha_c)$ \hfill {\em (see Eq.~\ref{eq:confidence-ellipsoids})} \\
    3. Observe $\;\mathcal{A}_t\;$ and construct the (estimated) safe policy set $\;\Pi_t$ \hfill {\em (see Eq.~\ref{eq:safe-policy-set})} \\
    4. Compute policy $\;(\pi_t,\widetilde{\theta}_t) = \argmax_{\pi \in \Pi_t,\;\theta \in \mathcal{C}_t^r(\alpha_r)} \mathbb{E}_{x \sim \pi}[ \langle x, \theta \rangle ]$\\
    5. Take action $\;x_t \sim \pi_t\;$ and observe reward and cost $\;(r_t,c_t)$
     }    
     \caption{Optimistic-Pessimistic Linear Bandit (OPLB)}
    \label{alg:optimistic-pessimistic-LB}
    \end{algorithm}
\end{minipage}
}

{\bf\em Line~1 of OPLB:} At each round $t\in[T]$, given the actions $\{x_s\}_{s=1}^{t-1}$, rewards $\{r_s\}_{s=1}^{t-1}$, and costs $\{c_s\}_{s=1}^{t-1}$ observed until the end of round $t-1$, OPLB first computes the $\ell_2$-regularized least-squares (RLS) estimates of $\theta_*$ and $\mu_*^{o,\perp}$ (projection of the cost parameter $\mu_*$ into the sub-space $\mathcal V_o^\perp$) as 

\vspace{-0.15in}
\begin{small}
\begin{equation}
\label{eq:param-est}
\widehat{\theta}_t = \Sigma_t^{-1} \sum_{s=1}^{t-1}r_sx_s, \qquad\quad \widehat{\mu}_t^{o,\perp} = (\Sigma_t^{o,\perp})^{-1}\sum_{s=1}^{t-1}c_s^{o,\perp}x_s^{o,\perp},    
\end{equation}
\end{small}
\vspace{-0.15in}

where $\lambda>0$ is the regularization parameter, and 

\vspace{-0.15in}
\begin{small}
\begin{align}
\label{eq:Sigmas}
&\Sigma_t = \lambda I + \sum_{s=1}^{t-1}x_sx_s^\top, \qquad\quad \Sigma_t^{o,\perp} = \lambda I_{\mathcal V_o^\perp} + \sum_{s=1}^{t-1}x_s^{o,\perp}(x_s^{o,\perp})^\top, \\ 
&c^{o,\perp}_t = c_t - \frac{\langle x_t,e_0\rangle}{\|x_0\|}c_0, \qquad\quad I_{\mathcal V_o^\perp} = I_{d\times d} - \frac{1}{\|x_0\|^2}x_0x_0^\top. 
\label{eq:proj-est}
\end{align}
\end{small}
\vspace{-0.15in}

In~\eqref{eq:Sigmas}, $\Sigma_t$ and $\Sigma_t^{o,\perp}$ are the Gram matrices of actions and projection of actions into the sub-space $\mathcal V_o^\perp$. Note that $\Sigma_t^{o, \perp}$ is a rank deficient matrix, but with abuse of notation, we use $(\Sigma_t^{o, \perp})^{-1}$ to denote its pseudo-inverse throughout the paper. In~\eqref{eq:proj-est}, $I_{\mathcal V_o^\perp}$ is the projection of the identity matrix, $I$, into $\mathcal V_o^\perp$, and $c^{o,\perp}_t$ is the noisy projection of the cost $c_t$ incurred by taking action $x_t$ into $\mathcal V_o^\perp$, i.e.,\footnote{In the derivation of~\eqref{eq:c-tilde-derivation}, we use the fact that $\langle x_t,\mu_*\rangle = \langle x_t^o+x_t^{o,\perp},\mu_*^o+\mu_*^{o,\perp}\rangle = \langle x_t^o,\mu_*^o\rangle + \langle x_t^{o,\perp},\mu_*^{o,\perp}\rangle$.}

\vspace{-0.15in}
\begin{small}
\begin{equation}
\label{eq:c-tilde-derivation}
c^{o,\perp}_t = \langle x_t^{o,\perp},\mu_*^{o,\perp}\rangle + \xi_t^c = \langle x_t,\mu_* \rangle - \langle x_t^o,\mu_*^o \rangle + \xi_t^c = c_t - \langle x_t^o,\mu_*^o \rangle = c_t - \frac{\langle x_t,e_0\rangle}{\|x_0\|}c_0.       
\end{equation}
\end{small}
\vspace{-0.125in}

{\bf\em Line~2:} Using the RLS estimates $\widehat{\theta}_t$ and $\widehat{\mu}_t^{o,\perp}$ in~\eqref{eq:param-est}, OPLB constructs the two {\em confidence sets} 

\vspace{-0.15in}
\begin{small}
\begin{equation}
\label{eq:confidence-ellipsoids}
\mathcal{C}_t^r(\alpha_r) = \big\{\theta \in \mathbb{R}^d: \|\theta -\widehat{\theta}_t\|_{\Sigma_t} \leq \alpha_r \beta_t(\delta, d)\big\}, \quad \mathcal{C}_t^c(\alpha_c) = \big\{ \mu \in \mathcal{V}_o^{\perp} : \| \mu - \widehat{\mu}^{o, \perp}_t\|_{\Sigma_t^{o,\perp}} \leq \alpha_c \beta_t(\delta, d-1)\big\},
\end{equation}
\end{small}
\vspace{-0.15in}

where $\alpha_r,\alpha_c\geq 1$ and $\beta_t(\delta,d)$ in the radii of these {\em confidence ellipsoids} is defined by the following theorem, originally proved in~\cite{abbasi2011improved}. 

\begin{theorem}\label{theorem::yasin_theorem}[Thm.~2 in~\citealt{abbasi2011improved}]
Let Assumptions~\ref{ass:noise-sub-gaussian} and~\ref{ass:bounded-reward-cost-param} hold, $\widehat{\theta}_t$, $\widehat{\mu}_t^{o,\perp}$, $\Sigma_t$, and $\Sigma_t^{o,\perp}$ defined by~\eqref{eq:param-est} and~\eqref{eq:Sigmas}, and $\mathcal{C}_t^r(\cdot)$ and $\mathcal{C}_t^c(\cdot)$ defined by~\eqref{eq:confidence-ellipsoids}. Then, for a fixed $\delta \in (0,1)$ and

\vspace{-0.1in}
\begin{small}
\begin{equation}
\label{eq:ellipsoid-radius}
\beta_t(\delta,d) = R \sqrt{d\log\Big(\frac{1 + (t-1)L^2/\lambda}{\delta}\Big)} + \sqrt{\lambda}\;S,
\end{equation}
\end{small}
\vspace{-0.125in}

with probability at least $1-\delta$ and for all $t \geq 1$, it holds that $\theta_*\in\mathcal{C}_t^r(1)$ and $\mu_*^{o,\perp}\in\mathcal{C}_t^c(1)$.
\end{theorem}

Since $\alpha_r,\alpha_c\geq 1$, for all rounds $t\in[T]$, the sets $\mathcal{C}_t^r(\alpha_r)$ and $\mathcal{C}_t^c(\alpha_c)$ also contain $\theta_*$, the reward parameter, and $\mu_*^{o,\perp}$, the projection of the cost parameter into $\mathcal V_o^\perp$, respectively, with high probability. 

Given these confidence sets, we define the {\em optimistic reward} and {\em pessimistic cost} of any policy $\pi$ in round $t$ as 

\vspace{-0.225in}
\begin{small}
\begin{equation}
\label{eq:max-reward-cost}
\widetilde{r}_{\pi,t} := \max_{\theta\in\mathcal{C}_t^r(\alpha_r)}   \mathbb{E}_{x \sim \pi}[\langle x,\theta\rangle], \qquad\qquad
\widetilde{c}_{\pi,t} := \frac{\langle x_{\pi}^o,e_0 \rangle c_0}{\| x_0 \|} + \max_{\mu\in\mathcal{C}_t^c(\alpha_c)} \mathbb{E}_{x\sim\pi}[\langle x,\mu \rangle].
\end{equation}
\end{small}
\vspace{-0.075in}

\begin{proposition}
\label{prop:optimistic-reward-pessimistic-cost}
We may write~\eqref{eq:max-reward-cost} in closed-form as \hfill {\em (proof in Appendix~\ref{subsec:proof-prop-optimistic-reward})}

\vspace{-0.15in}
\begin{small}
\begin{align}
\label{eq:optimistic-reward-closed-form}
\widetilde{r}_{\pi,t} &= \langle x_\pi,\widehat{\theta}_t \rangle + \alpha_r \beta_t(\delta,d) \| x_\pi\|_{\Sigma_t^{-1}}, \\ \widetilde{c}_{\pi,t} &= \frac{\langle x_\pi^o, e_0\rangle c_0 }{\|x_0\|} + \langle x_\pi^{o, \perp}, \widehat{\mu}^{o, \perp}_t \rangle + \alpha_c \beta_t(\delta,d-1) \| x_{\pi}^{o, \perp}\|_{(\Sigma_t^{o, \perp})^{-1}}.
\label{eq:pessimistic-cost-closed-form}
\end{align}
\end{small}
\vspace{-0.15in}

\end{proposition}

%It is easy to see that $\widetilde{r}_{\pi,t}=\langle x_\pi,\widehat{\theta}_t \rangle + \alpha_r \beta_t(\delta,d) \| x_\pi\|_{\Sigma_t^{-1}} $ and $\widetilde{c}_{\pi,t} = \frac{\langle x_\pi^o, e_0\rangle c_0 }{\|x_0\|} + \langle x_\pi^{o, \perp}, \widehat{\mu}^{o, \perp}_t \rangle + \alpha_c \beta_t(\delta,d-1) \| x_{\pi}^{o, \perp}\|_{(\Sigma_t^{o, \perp})^{-1}} $. %The discrepancy between the definitions of $\tilde{V}_t^r$ and $\tilde{V}_t^c$ has been introduced to take into account the knowledge of $\langle x_0, \mu^* \rangle$. \mgh{I do not understand what you mean by the last sentence. Remove it if it is redundant.}

{\bf\em Line~3:} After observing the action set $\mathcal A_t$, OPLB constructs its (estimated) feasible (safe) policy set

\vspace{-0.15in}
\begin{small}
\begin{equation}
\label{eq:safe-policy-set}
\Pi_t = \{\pi \in \Delta_{\mathcal A_t} : \widetilde{c}_{\pi,t} \leq \tau\}, 
%\Pi_t = \big\{\pi \in \Delta_{\mathcal A_t} :\frac{\langle x_\pi^o, e_0\rangle c_0 }{\|x_0\|} + \langle x_\pi^{o, \perp}, \widehat{\mu}^{o, \perp}_t \rangle + \alpha_c \beta_t(\delta,d-1) \| x_{\pi}^{o, \perp}\|_{(\Sigma_t^{o, \perp})^{-1}}  \leq \tau \big\}.
\end{equation}
\end{small}
\vspace{-0.175in}

where $\widetilde{c}_{\pi,t}$ is the pessimistic cost of policy $\pi$ in round $t$ defined by~\eqref{eq:pessimistic-cost-closed-form}. Note that $\Pi_t$ is not empty since $\pi_0$, the policy that plays the safe action $x_0$ with probability (w.p.)~$1$, is always in $\Pi_t$. This is because $x_{\pi_0}^o = x_0$, $x_{\pi_0}^{o,\perp} =0$, and $\frac{\langle x_{\pi_0}^o, e_0\rangle c_0}{\| x_0 \|}  = c_0$. In the following proposition, whose proof is reported in Appendix~\ref{subsec:proof-safe-set}, we prove that all policies in $\Pi_t$ are feasible with high probability.

\begin{proposition}
\label{prop:safe-set}
With probability at least $1-\delta$, for all rounds $t\in[T]$, all policies in $\Pi_t$ are feasible. %\aldo{Get this in}
\end{proposition}

{\bf\em Line~4:} The agent computes its policy, $\pi_t$, as the one that is safe (belongs to $\Pi_t$) and attains the maximum optimistic reward. We refer to $\widetilde{\theta}_t$ as the {\em optimistic reward parameter}. Thus, we write the optimistic reward of policy $\pi_t$ as $\widetilde{r}_{\pi_t,t} = \langle x_{\pi_t},\widetilde{\theta}_t \rangle$.

{\bf\em Line~5:} Finally, the agent selects an action $x_t\sim\pi_t$ and observes the reward-cost pair $(r_t,c_t)$.

{\bf Computational Complexity of OPLB.} $\;$ As shown in Line~4 of Algorithm~\ref{alg:optimistic-pessimistic-LB} and in Proposition~\ref{prop:optimistic-reward-pessimistic-cost}, in each round $t$, OPLB solves the following optimization problem:

\vspace{-0.15in}
\begin{small}
\begin{align}
\label{equation::opt_problem_linear}
\max_{\pi \in \Delta_{\mathcal{A}_t}}&  \langle x_\pi, \widehat{\theta}_t \rangle + \alpha_r \beta_t(\delta,d) \| x_\pi\|_{\Sigma_t^{-1}} \\ %\tag{OPT} \\
\text{s.t. }&   \frac{\langle x_\pi^o, e_0\rangle c_0 }{\|x_0\|} + \langle x_\pi^{o, \perp}, \widehat{\mu}^{o, \perp}_t \rangle + \alpha_c \beta_t(\delta,d-1) \| x_{\pi}^{o, \perp}\|_{(\Sigma_t^{o, \perp})^{-1}} \leq \tau. \nonumber
\end{align}
\end{small}
\vspace{-0.15in}

However, solving~\eqref{equation::opt_problem_linear} can be challenging. The bottleneck is computing the safe policy set $\Pi_t$, which is the intersection between $\Delta_{\mathcal{A}_t}$ and the ellipsoidal constraint.
%since computing the intersection of the . The principal computational bottleneck is the difficulty of computing and getting an adequate handle of the intersection between $\Delta_{\mathcal{A}_t}$ and the ellipsoidal constraints. Since the objective function is the same as in LinUCB (\cite{abbasi2011improved}), our algorithm has the same computational complexity of LinUCB whenever the feasible policy sets $\Pi_t$ (all of which are convex) can be represented in a form that admits optimization of the LinUCB objective. 
%We provide tractable (polynomial time) algorithms for \ref{equation::opt_problem_linear} in the special cases when $\mathcal{A}_t$ is convex and when $\mathcal{A}_t$ is a finite set. The details are in the Appendix. %\aldo{Check this}

\begin{remark}
The main challenge in obtaining a regret bound for OPLB is to ensure that optimism holds in each round $t$, i.e.,~the solution $(\pi_t,\widetilde\theta_t)$ of~\eqref{equation::opt_problem_linear} satisfy $\widetilde{r}_{\pi_t,t} = \langle x_{\pi_t},\widetilde\theta_t \rangle \geq r_{\pi^*_t}$. This is not obvious, since the (estimated) safe policy set $\Pi_t$ may not contain the optimal policy $\pi_t^*$. Our main algorithmic innovation is the use of asymmetric confidence intervals $\mathcal{C}_t^r(\alpha_r)$ and $\mathcal{C}_t^c(\alpha_c)$ for $\theta_*$ and $\mu^{o, \perp}_*$, which allows us to guarantee optimism, by appropriately selecting the ratio $\gamma = \alpha_r/\alpha_c$. Of course, this comes at the cost of scaling the regret by a factor $\gamma$. As it will be shown in our analysis in Section~\ref{section::lin_opt_pess_analysis}, $\gamma$ depends on the inverse gap $1/(\tau-c_0)$, which indicates when $\tau - c_0$ is small (the cost of the safe arm is close to the constraint threshold), the agent will have a difficult time to identify a safe arm and to compete against the optimal feasible policy $\pi_t^*$. We will formalize this in Lemma \ref{lemma:linear_bandits_optimism}. 
\end{remark}

\begin{remark}%[Unknown $c_0$]
If the cost of the safe arm $c_0$ is unknown, we start by taking the safe action $x_0$ for $T_0$ rounds to produce a conservative estimate $\hat\delta_c$ of $\tau - c_0$ that satisfies $\hat\delta_c \geq \frac{\tau - c_0}{2}$. We warm start our estimators for $\theta_*$ and $\mu_*$ using the data collected by playing $x_0$. However, instead of estimating $\mu_*^{o, \perp}$, we build an estimator for $\mu_*$ over all its directions, including $e_0$, similar to what OPLB does for $\theta_*$. We then set $\frac{\alpha_r}{\alpha_c} = 1/\hat\delta_c$ and run Algorithm~\ref{alg:optimistic-pessimistic-LB} for rounds $t > T_0$ (see Appendix~\ref{section::safe_policy_value} for more details). 
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Regret Analysis}
\label{section::lin_opt_pess_analysis}

In this section, we prove the following regret bound for OPLB (Algorithm~\ref{alg:optimistic-pessimistic-LB}). 

\begin{theorem}[Regret of OPLB]
\label{theorem::main_theorem_linear}
Let $\alpha_c = 1$ and $\alpha_r = \frac{ 2+\tau-c_0}{\tau-c_0}$. Then, with probability at least $1-2\delta$, the regret of OPLB satisfies %\mgh{Let's see if we get rid of $\gamma$ later.}

\vspace{-0.15in}
\begin{small}
\begin{equation}
\label{eq:regret-OPLB}
\mathcal{R}_{\Pi}(T) \leq \frac{2L(\alpha_r+1)\beta_T(\delta, d)}{\sqrt{\lambda}}\sqrt{2T\log(1/\delta)} + (\alpha_r+1)\beta_T(\delta, d)\sqrt{2Td\log(1+\frac{TL^2}{\lambda})}.
\end{equation}
\end{small}
\vspace{-0.15in}
\end{theorem}

We start the proof of Theorem~\ref{theorem::main_theorem_linear}, by defining the following event that holds w.p.~at least $1-\delta$: 

\vspace{-0.125in}
\begin{small}
\begin{equation}
\label{eq:high-prob-event}
\mathcal{E} := \big\{\|\widehat{\theta}_t - \theta_*\|_{\Sigma_t} \leq \beta_t(\delta, d) \; \wedge \; \|\widehat{\mu}_t^{o, \perp} - \mu_*^{o, \perp}\|_{\Sigma_t^{o,\perp}} \leq \beta_t(\delta, d-1), \; \forall t\in[T]\big\}.
\end{equation}
\end{small}
\vspace{-0.15in}

The regret $\mathcal{R}_{\Pi}(T)$ in~\eqref{eq:regret} can be decomposed as ($\widetilde{r}_{\pi_t,t}$ is the optimistic reward defined by Eq.~\ref{eq:max-reward-cost})

\vspace{-0.15in}
\begin{small}
\begin{equation}
\label{eq:regret-decomp}
\mathcal{R}_{\Pi}(T) = \underbrace{\sum_{t=1}^T r_{\pi_t^*} - \widetilde{r}_{\pi_t,t}}_{(\mathrm{I})} \; + \; \underbrace{\sum_{t=1}^T \widetilde{r}_{\pi_t,t} - r_{\pi_t}}_{(\mathrm{II})}.
\end{equation}
\end{small}
\vspace{-0.125in}

We first bound the term $(\mathrm{II})$ in~\eqref{eq:regret-decomp}. To bound $(\mathrm{II})$, we further decompose it as

\vspace{-0.15in}
\begin{small}
\begin{equation}
\label{eq:II-decomp}
(\mathrm{II}) = \underbrace{\sum_{t=1}^T  \langle x_{\pi_t}, \widetilde{\theta}_t \rangle - \langle x_t, \widetilde{\theta}_t \rangle}_{(\mathrm{III})} + \underbrace{\sum_{t=1}^T \langle x_t, \widetilde{\theta}_t \rangle - \langle x_t, \theta_* \rangle}_{(\mathrm{IV})} + \underbrace{\sum_{t=1}^T \langle x_t, \theta_* \rangle - \langle x_{\pi_t}, \theta_* \rangle }_{(\mathrm{V})}.
\end{equation}
\end{small}
\vspace{-0.125in}

In the following lemmas, we first bound the sum of $(\mathrm{III})$ and $(\mathrm{V})$ terms, and then bound $(\mathrm{IV})$.

\begin{lemma}
\label{lemma:bounding-3+5}
On the event $\mathcal{E}$ defined by~\eqref{eq:high-prob-event}, for any $\gamma \in (0, 1)$, w.p.~at least $1-\gamma$, we have

\vspace{-0.125in}
\begin{small}
\begin{equation*}
(\mathrm{III}) + (\mathrm{V}) \leq \frac{2L(\alpha_r + 1)\beta_T(\delta, d)}{\sqrt{\lambda}}\cdot\sqrt{2 T \log(1/\gamma)}\;.
\end{equation*}
\end{small}
\end{lemma}

\vspace{-0.175in}
\begin{proof}
We write $(\mathrm{III}) + (\mathrm{V}) = \sum_{t=1}^T \langle x_{\pi_t} - x_t, \widetilde{\theta}_t - \theta_* \rangle$. By Cauchy-Schwartz, we have $|\langle x_{\pi_t} - x_t, \widetilde{\theta}_t - \theta_* \rangle | \leq \| x_{\pi_t} - x_t \|_{\Sigma^{-1}_t} \| \widetilde{\theta}_t - \theta_*\|_{\Sigma_t}$. Since $\widetilde{\theta}_t\in \mathcal{C}_t^r(\alpha_r)$, on event $\mathcal E$, we have $\|\widetilde{\theta}_t - \theta_*\|_{\Sigma_t} \leq (\alpha_r+1) \beta_t(\delta, d)$. Also from the definition of $\Sigma_t$, we have $\Sigma_t \succeq \lambda I$, and thus, $\| x_{\pi_t} - x_t \|_{\Sigma^{-1}_t} \leq \| x_{\pi_t} - x_t\|/\sqrt{\lambda} \leq 2L/\sqrt{\lambda}$. Therefore, $Y_t =\sum_{s=1}^t \langle x_{\pi_s} - x_s, \widetilde{\theta}_s - \theta_* \rangle$ is a martingale sequence with $|Y_t - Y_{t-1}| \leq 2L(\alpha_r + 1)\beta_t(\delta, d)/\sqrt{\lambda}$, for $t\in [T]$. By the Azuma–Hoeffding inequality and since $\beta_t$ is an increasing function of $t$, i.e.,~$\beta_t(\delta, d) \leq \beta_T(\delta, d),\;\forall t\in[T]$, w.p.~at least  $1-\gamma$, we have $\mathbb{P}\big(Y_T \geq 2L(\alpha_r + 1) \beta_T(\delta, d)\sqrt{2T \log(1/\gamma)/\lambda}\big) \leq \gamma$, which concludes the proof. 
\end{proof}

\begin{lemma}
\label{lemma:bounding-4}
On event $\mathcal{E}$, we have $(\mathrm{IV}) \leq (\alpha_r+1) \beta_T(\delta,d)\sqrt{2Td\log\big(1+\frac{TL^2}{\lambda}\big)}$. \end{lemma}

We report the proof of Lemma~\ref{lemma:bounding-4} in Appendix~\ref{subsec:proof-Lemma-bounding-4}. After bounding all the terms in $(\mathrm{II})$, we now process the term $(\mathrm{I})$ in~\eqref{eq:regret-decomp}. Before stating the main result for this term  in Lemma~\ref{lemma:linear_bandits_optimism}, we need to prove the following lemma (proof in Appendix~\ref{subsec:proof-Lemma-inverse-norm-domination}). 
\begin{lemma}
\label{lemma:inverse_norm_domination}

For any policy $\pi$, the following inequality holds: 

\vspace{-0.125in}
\begin{small}
\begin{equation}
\label{equation::comparison_conf_bounds}
\| x_\pi^{o, \perp}\|_{(\Sigma_t^{o,\perp})^{-1}} \leq \| x_\pi \|_{\Sigma_t^{-1}}.
\end{equation}
\end{small}
\end{lemma}

In the following lemma, we prove that by appropriately setting the parameters $\alpha_r$ and $\alpha_c$, we can guarantee that at each round $t\in[T]$, OPLB selects an optimistic policy, i.e.,~a policy $\pi_t$, whose optimistic reward, $\widetilde{r}_{\pi_t,t}$, is larger than the reward of the optimal policy $r_{\pi^*_t}$, given the event $\mathcal E$. This means that with our choice of parameters $\alpha_r$ and $\alpha_c$, the term $(\mathrm{I})$ in~\eqref{eq:regret-decomp} is always non-positive.

\begin{lemma}
\label{lemma:linear_bandits_optimism}
On the event $\mathcal{E}$, if we set $\alpha_r$ and $\alpha_c$, such that $\alpha_r,\alpha_c\geq 1$ and $1+\alpha_c \leq (\tau-c_0) (\alpha_r-1)$, then for any $t\in[T]$, we have $\widetilde{r}_{\pi_t,t} \geq r_{\pi_t^*}$.
\end{lemma}

Here we provide a proof sketch for Lemma~\ref{lemma:linear_bandits_optimism}. The detailed proof is reported in Appendix~\ref{subsec:proof-Lemma-term-I}. 

\begin{proof}[Proof Sketch]
We divide the proof into two cases, depending on whether in each round $t$, the optimal policy $\pi^*_t$ belongs to the (estimated) set of feasible policies $\Pi_t$, or not. 

{\bf Case~yes
1.} $\;$ If $\pi_t^*\in\Pi_t$, then its optimistic reward is less than that of the policy $\pi_t$ selected at round $t$ (by the definition of $\pi_t$ on Line~4 of Algorithm~\ref{alg:optimistic-pessimistic-LB}), i.e.,~$\widetilde{r}_{\pi_t^*,t}\leq\widetilde{r}_{\pi_t,t}$. This together with the fact that the optimistic reward of any policy $\pi$ is larger than its expected reward, i.e.,~$\widetilde{r}_{\pi,t}\geq r_\pi$, gives us the desired result that $\widetilde{r}_{\pi_t,t}\geq r_{\pi^*_t}$. 

{\bf Case~2.} $\;$ If $\pi_t^*\not\in\Pi_t$, then we define a mixture policy $\widetilde{\pi}_t=\eta_t\pi_t^*+(1-\eta_t)\pi_0$, where $\pi_0$ is the policy that always selects the safe action $x_0$ and $\eta_t\in[0,1]$ is the maximum value of $\eta$ for which the mixture policy belongs to the set of feasible actions, i.e.,~$\widetilde{\pi}_t\in\Pi_t$. Conceptually, we can think of $\eta_t$ as a measure for safety of the optimal policy $\pi_t^*$. Mathematically, $\eta_t$ is the value at which the pessimistic cost of the mixture policy equals to the constraint threshold, i.e.,~$\widetilde{c}_{\widetilde{\pi}_t,t} =\tau$. In the rest of the proof, we first write $\widetilde{c}_{\widetilde{\pi}_t,t}$ in terms of the pessimistic cost of the optimal policy as $\widetilde{c}_{\widetilde{\pi}_t,t}=(1-\eta_t)c_0+\eta_t\widetilde{c}_{\pi^*_t,t}$ ($c_0$ is the expected cost of the safe action $x_0$), and find a lower-bound for $\eta_t$ (see Eq.~\ref{eq:tempB3} in Appendix~\ref{subsec:proof-Lemma-term-I}). We then use the fact that since $\widetilde{\pi}_t\in\Pi_t$, its optimistic reward is less than that of $\pi_t$, i.e.,~$\widetilde{r}_{\pi_t,t}\geq \widetilde{r}_{\widetilde{\pi}_t,t}$, and obtain a lower-bound for  $\widetilde{r}_{\widetilde{\pi}_t,t}$ as a function of $r_{\pi_t^*}$ (see Eq.~\ref{eq:tempB4} in Appendix~\ref{subsec:proof-Lemma-term-I}). Finally, we conclude the proof by using this lower-bound and finding the relationship between the parameters $\alpha_r$ and $\alpha_c$ for which the desired result $\widetilde{r}_{\pi_t,t}\geq r_{\pi_t^*}$ is obtained, i.e.,~$1+\alpha_c\leq (\tau-c_0)(\alpha_r-1)$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{theorem::main_theorem_linear}]
The proof follows from the fact that the term $(\mathrm{I})$ is negative (Lemma~\ref{lemma:linear_bandits_optimism}), and by combining the upper-bounds on the term $(\mathrm{II})$ from Lemmas~\ref{lemma:bounding-3+5} and~\ref{lemma:bounding-4}, and setting $\gamma = \delta$.
\end{proof}




%We can combine the results of Lemmas \ref{lemma::bounding_A_C} and \ref{lemma::bounding_B} to obtain the main theorem of this section:


% \begin{proof}
% The result follows immediately as a consequence of the previous results.
% \end{proof}


% \subsection{Multiple Linear Constraints}

% The exact same argument as in the multi armed bandits case will apply here. 






























==> Constrained Bandits/lower_bounds.tex <==
We start by proving a generalized version of the divergence decomposition lemma for bandits. %We follow the template from \cite{lattimore2018bandit}:

\begin{lemma}\label{lemma::divergence_decomposition}[Divergence decomposition for constrained multi armed bandits] Let $\nu = ((P_1, Q_1), \cdots, (P_K, Q_K))$ be the reward and constraint distributions associated with one instance of the single constraint multi-armed bandit, and let $\nu' = ((P_1', Q_1'), \cdots, (P_K', Q_K'))$ be the reward and constraint distributions associated with another constrained bandit instance. Fix some algorithm $\mathcal{A}$ and let $\mathbb{P}_\nu = \mathbb{P}_{\nu^\mathcal{A}}$ and $\mathbb{P}_{\nu'} = \mathbb{P}_{\nu'^\mathcal{A}}$ be the probability measures on the cannonical bandit model (See section 4.6 of \cite{lattimore2018bandit}) induced by the $T$ round interconnection of $\mathcal{A}$ and $\nu$ (respectively $\mathcal{A}$ and $\nu'$). Then:
\begin{equation*}
    \mathrm{KL}(\mathbb{P}_\nu, \mathbb{P}_{\nu'}) = \sum_{a=1}^K \mathbb{E}_{\nu}[T_a(T)] \mathrm{KL}((P_a,Q_a), (P_a', Q_a'))
\end{equation*}
Where $T_a(T)$ denotes the number of times arm $a$ was pulled until by $\mathcal{A}$ and up to time $T$. 
\end{lemma}

\begin{proof}
The same proof as in Lemma 15.1 from \cite{lattimore2018bandit} applies in this case. 
\end{proof}

The following two lemmas will prove useful as well:

\begin{lemma}\label{lemma::gaussian_divergence}[Gaussian Divergence ] The divergence between two multivariate normal distributions and means $\mu_1, \mu_2 \in \mathbb{R}^d$ with spherical identity covariance $\mathbb{I}_d$ equals:
\begin{equation*}
    \mathrm{KL}(\mathcal{N}(\mu_1, \mathbb{I}_d) , \mathcal{N}(\mu_2, \mathbb{I}_d) ) = \frac{\| \mu_1- \mu_2\|^2 }{2}
\end{equation*}
\end{lemma}

Define the binary relative entropy to be:
\begin{equation*}
    d(x,y) = x\log(\frac{x}{y}) + (1-x) \log( \frac{1-x}{1-y})
\end{equation*}
and satisfies:
\begin{equation}\label{equation::lower_bound_divergence}
d(x,y) \geq (1/2)\log(1/4y)
\end{equation}
for $x \in [1/2,1]$ and $y \in (0,1)$.
Adapted from~\cite{kaufmann2016complexity}, Lemma 1.
\begin{lemma}\label{lemma::binary_relative_entropy}
Let $\nu, \nu'$ be two constrained bandit models with $K$ arms. Borrow the setup, definitions and notations of Lemma~\ref{lemma::divergence_decomposition}, then for any measurable event $\mathcal{B} \in \mathcal{F}_T$:
\begin{equation}\label{equation::relative_entropy_bound}
   \mathrm{KL}(\mathbb{P}_\nu, \mathbb{P}_{\nu'}) =\sum_{a=1}^K \mathbb{E}_{\nu}[T_a(T)] \mathrm{KL}((P_a,Q_a), (P_a', Q_a')) \geq d(\mathbb{P}_\nu( \mathcal{B})  , \mathbb{P}_{\nu'}(\mathcal{B} ))
\end{equation}
\end{lemma}


% \begin{theorem}\label{lemma::bretagnole_huber}[Bretagnolle-Huber] Let $P$ and $Q$ be probability measures on the same measurable space $(\Omega, \mathcal{F})$ and let $A \in \mathcal{F}$ be an arbitrary event. Then:
% \begin{equation*}
% P(A) + Q(A^c) \geq \frac{1}{2}\exp\left( -D(P,Q)\right)
% \end{equation*}
%  Where $A^c = \Omega \backslash A$ is the complement of $A$.
% \end{theorem}

We now present a worst-case lower bound for the constrained multi armed bandit problem. We restrict ourselves to Gaussian instances with mean reward and cost vectors $\bar{r}, \bar{c} \in [0,1]^K$. Let $\mathcal{A}$ be an algorithm for policy selection in the constrained MAB problem.  For the purpose of this section
we denote as $\mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}, \bar{c} )$ as the constrained regret of algorithm $\mathcal{A}$ in the Gaussian instance $\mathcal{N}(\bar{r}, \mathbb{I})$, $\mathcal{N}( \bar{c}, \mathbb{I})$. The following theorem holds:


\begin{theorem}
Let $\tau, \bar{c}_1 \in (0,1)$, $K \geq 4$, and $B:=\max\left(\frac{1}{27}\sqrt{ (k-1) T}, \frac{1}{6(\tau - \bar{c}_1)^2} \right)$  and assume\footnote{This constraint on $T$ translates to $T \geq C$ for some constant $C$.} $T \geq \max(  K-1,24eB)$ and let $\tau$ be the maximum allowed cost. Then for any algorithm $\mathcal{A}$ there is a pair of mean vectors $\bar{r}, \bar{c} \in [0,1]^K$ such that:
\begin{equation*}
    \mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}, \bar{c}) \geq B
\end{equation*}
\end{theorem}
\begin{proof}

%We start with the assumption that $\frac{1}{\tau - \bar{c}_1} =o( \sqrt{T}  )$. 
If $\max\left(\frac{1}{27}\sqrt{ (k-1) T}, \frac{1}{6(\tau - \bar{c}_1)^2} \right) = \sqrt{KT}$, then the argument in Theorem 15.2 of \cite{lattimore2018bandit} yields the desired result by noting that the framework of constrained bandits subsumes unconstrained multi armed bandits when all costs equal zero. In this case we conclude there is an instance $\bar{r}, \bar{c}$ with $\bar{c}_a =0$ for all $a \in \mathcal{A}$ satisfying:
\begin{equation*}
    \mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}, \bar{c}) \geq \frac{1}{27}\sqrt{ (k-1) T}
\end{equation*}

Let's instead focus on the case where $B = \max\left(\frac{1}{27}\sqrt{ (k-1) T}, \frac{1}{6(\tau - \bar{c}_1)^2} \right) =\frac{1}{6(\tau - \bar{c}_1)^2} $.

Pick any algorithm. We want to show that the algorithm's regret on some environment is as large as $B$. If there was an instance $\bar{r}, \bar{c}$ such that $\mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}, \bar{c}) > B$ there would be nothing to be proven. Hence without loss of generality, we can assume that the algorithm satisfies $\mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}, \bar{c}) \leq B $ for all $\bar{r}, \bar{c} \in [0,1]^K$ and having unit variance Gaussian rewards. 

Let $c \in (0,1)$ with $c =  \tau-\bar{c}_1$. For the reader's convenience we will use the notation $\Delta = 1/2$. By treating the rewards in a symbolic way it is easier to understand the logic of the proof argument. Let's consider the following constrained bandit instance inducing measure $\nu$:
\begin{align*}
    \bar{c}^1  &= (\tau - c, &\tau+2c,&\quad \tau-c,& \tau+2c, &\quad\cdots,& \tau+2c )\\
    \bar{r}^1 &= (\Delta,& 8\Delta,&\quad 0, &4\Delta,&\quad \cdots, &4\Delta)
\end{align*}

Notice that the optimal policy equals a mixture between arm $1$ and $2$, where arm $1$ is chosen with probability $2/3$ and arm 2 with probability $1/3$. The value of this optimal policy equals $10/3\Delta$. 

Recall we use the notation $\bar{T}_j(t)$ denote the total amount of probability mass that $\mathcal{A}$ allocated to arm $j$ up to time $t$. Notice that the expected reward of all feasible policies that do not have arm $1$ in their support have a gap (w.r.t the optimal feasible policy's expected reward) of at least $\frac{2\Delta}{3}$. Since by assumption, $\mathcal{A}$ satisfies $\mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}^1, \bar{c}^1) \leq B $:
\begin{align*}
   B &\geq \mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}^1,\bar{c}^1) &\geq\frac{2\Delta}{3} \left( \frac{2}{3}T - \frac{1}{2}T \right) \mathbb{P}\left( \bar{T}_1(T) < \frac{T}{2}  \right)   & = \frac{\Delta}{9}T \mathbb{P}\left( \bar{T}_1(T) < \frac{T}{2}  \right)
\end{align*}
And therefore:
\begin{align*}
    \mathbb{P}\left( \bar{T}_1(T) \geq \frac{T}{2} \right) = 1-\mathbb{P}\left(  \bar{T}_1(T) < \frac{T}{2}  \right) \geq 1-\frac{9B}{\Delta T} \geq 1/2
\end{align*}
The last inequality follows from the assumption $T \geq \max(  K-1,24eB)$.%  \aldo{Explain better why this is $2/3T - 1/2T$}

% Suppose $\mathcal{A}$ satisfies a sublinear regret guarantee for all constrained instances. In other words, let's assume  there exists $\alpha \in (0,1)$ such that:

% \begin{equation}\label{equation::sublinear_regret}
%     \mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}_1, \bar{c}_1) \leq C T^{\alpha} 
% \end{equation}
% For some universal constant $C$. Notice that the only feasible policy achieving the optimum plays arm $1$ with probability $2/3$, way larger than $1/2$ . All other feasible policies achieve a value that is at least $4/3\Delta$ away from $10/3\Delta$, the value of the optimal policy. Let $T$ be large enough so that:
% \begin{equation}
% \mathbb{P}(T_1 \geq \frac{T}{2}) \geq 1/2
% \end{equation}
% This is possible because by the assumption in Equation \ref{equation::sublinear_regret} which in turn implies arm $1$ should be picked very often with a mixture weight of at least $2/3$ the majority of the time, except perhaps a "sublinear" amount of time.

Let's now consider the following constrained bandit instance inducing measure $\nu'$:
\begin{align*}
    \bar{c}_2 &= (\tau - c, &\tau+2c,&\quad 0,& \tau-c, &\quad\cdots,& \tau+2c )\\
    \bar{r}_2 &= (\Delta,& 8\Delta,&\quad 0, &4\Delta,&\quad \cdots, &4\Delta)
\end{align*}
In this instance the optimal policy is to play arm 4 deterministically, which gets a reward of $4\Delta$. Notice that the expected reward of any feasible policy that does not contain arm $4$ in its support has a gap (w.r.t. the optimal feasible policy's expected reward) of at least $\frac{2\Delta }{3}$. Since by assumption, $\mathcal{A}$ satisfies $\mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}^2, \bar{c}^2) \leq B $:
\begin{align*}
    B &\geq \mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}^2, \bar{c}^2) &\geq\frac{2\Delta}{3} \left(  \frac{1}{2}T \right) \mathbb{P}\left( \bar{T}_1(T) \geq \frac{T}{2}  \right)   & = \frac{\Delta}{3}T \mathbb{P}\left( \bar{T}_1(T) \geq \frac{T}{2}  \right)
\end{align*}
And therefore:
\begin{equation*}
    \mathbb{P}\left( \bar{T}_1(T) \geq \frac{T}{2} \right) \leq \frac{3B}{\Delta T} \leq \frac{1}{4e}
\end{equation*}
The last inequality follows from the assumption $T \geq \max(  K-1,24eB)$. As a consequence of inequality~\ref{equation::lower_bound_divergence}, Lemma~\ref{lemma::binary_relative_entropy} and~\ref{lemma::gaussian_divergence}:
\begin{equation*}
    \mathbb{E}_\nu[T_4(T)]\mathrm{KL}(\binom{\tau+2c}{4\Delta}, \mathbb{I}_d) , \mathcal{N}(\binom{\tau-c}{4\Delta}, \mathbb{I}_d) ) = \mathbb{E}_\nu[T_4(T)]2c^2 \geq \frac{1}{2}
\end{equation*}
And therefore we can conclude:
\begin{equation}
 \mathbb{E}[\bar{T}_4(T)]= \mathbb{E}[T_4(T)]  \geq \frac{1}{4c^2}
\end{equation}
Since in $\nu$, any feasible policy with support in arm $4$ and no support in arm 2 has a suboptimality gap of $4/3\Delta$, we conclude the regret $\mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}^2, \bar{c}^2)$ must satisfy:
\begin{equation*}
    \mathcal{R}_\Pi(T, \mathcal{A}, \bar{r}^2, \bar{c}^2) \geq \frac{\Delta}{3c^2} 
\end{equation*}
Since $\Delta= \frac{1}{2}$ and noting that in this case $\frac{\Delta}{3c^2} = B$. The result follows. 
\end{proof}







% \begin{theorem}
% Let $K > 1 $ and $T \geq K-1$. Then, for any algorithm $\mathcal{A}$, there is a pair of mean vectors $\bar{r}, \bar{c} \in [0,1]^K$ such that (where $c_0 = 0$ and $\tau$):
% \begin{equation*}
%     \mathcal{R}_\Pi(T) \geq \frac{1}{27} \sqrt{ }
% \end{equation*}
% \end{theorem}

% \begin{proof}
% Fix algorithm $\mathcal{A}$. Let $\Delta \in [0,1/2], 1 \leq b \leq a \leq \frac{1}{\tau}$ be come constants that will be chosen later. We start with a constrained Gaussian bandit instance with unit variances and mean rewards $\bar{r} = (\Delta, 2\Delta, \cdots, 2\Delta)$ and costs $\bar{c} = (0, a\tau, \cdots, a\tau)$. This environment gives rise to the distribution $\mathbb{P}_{\nu_{\bar{r}, \bar{c}}, \mathcal{A}}$ in the cannonical bandit model. For brevity we will use $\mathbb{P}_{\bar{r}, \bar{c}}$ instead of $\mathbb{P}_{\nu_{\bar{r}, \bar{c}}, \mathcal{A}}$, and expectations under $\mathbb{P}_{\bar{r}, \bar{c}}$ will be denoted by $\mathbb{E}_{\bar{r}, \bar{c}}$. 

% Let's index the arms from $0$ to $K-1$. We assume arm $0$ is the safe arm with known cost $0$ and unknown mean reward $\Delta$. Let $\pi_1, \cdots, \pi_T$ be the policies proposed by $\mathcal{A}$ during the run of the algorithm. For any $i \in \{ 0, \cdots K-1\}$ let $\tilde{T}_i = \sum_{t=1}^T \pi_t(i)$ be the total mass allocated by $\mathcal{A}$ to action $i$. 

% Let $i = \arg\min_{j> 0} \mathbb{E}_{\bar{r}, \bar{c}} [ \tilde{T}_j(T)]$. Notice that any feasibile policy $\pi_t$ satisfies $\pi_t(j) \leq \frac{1}{a}$, and therefore since $\sum_{j=1}^K \tilde{T}_j(T) = T$:
% \begin{equation*}
%     \mathbb{E}_{\bar{r}, \bar{c}}[ \tilde{T}_i(T)  ] \leq \frac{T}{a(K-1) } 
% \end{equation*}
% Furthermore, since for all $j\in \{0, \cdots, K-1\}$ it follows that $\mathbb{E}_{\bar{r}, \bar{c}}[T_j(T)] =  \mathbb{E}_{\bar{r}, \bar{c}}[\tilde{T}_j(T)] $, we conclude that:
% \begin{equation}\label{equation::upper_bound_T_i}
%     \mathbb{E}_{\bar{r}, \bar{c}}[ T_i(T)  ] \leq \frac{T}{a(K-1) } 
% \end{equation}
% Let's build a second constrained  Gaussian bandit instance with unit variances and mean rewards $\bar{r}' = (\Delta, 2\Delta, \cdots, 2\Delta, 2\Delta,\cdots, 2\Delta)$ and costs $\bar{c}'= (0, a\tau, \cdots, b\tau, \cdots, a\tau)$ where specifically $\bar{c}'_i = b\tau$. Therefore $\bar{r}_j = \bar{r}_j'$ for all $j$ and $\bar{c}_j  = \bar{c}_j'$ except at index $i$. Let $\mathbb{P}_{\bar{r}', \bar{c}'}$ be the distribution induced by environment $\bar{r}', \bar{c}'$. The optimal policy $\pi^{*}$ for $\mathbb{P}_{\bar{r}, \bar{c}}$ is to play the mixture policy that selects arm $0$ with probability $1-\frac{1}{a}$ and any arm $j > 0$ with probability $\frac{1}{a}$. The optimal policy $\underline{\pi}^{*}$ for $\mathbb{P}_{\bar{r}', \bar{c}'}$ is to play the mixture policy that selects arm $0$ with probability $1-\frac{1}{b}$ and arm $i$ with probability $\frac{1}{b}$. Policy $\pi^*$ has value $\Delta + \frac{\Delta}{a}$ in $\mathbb{P}_{\bar{r}, \bar{c}}$ and policy $\underline{\pi}^{*}$ has value $\Delta + \frac{\Delta}{b}$ in $\mathbb{P}_{\bar{r}', \bar{c}'}$. A simple calculation leads to:
% \begin{align*}
%     \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}, \bar{c})&\geq \mathbb{P}_{\bar{r}, \bar{c}}\left( \tilde{T}_0(T) \leq T - \frac{T}{2b} + \frac{T}{2a}    \right) \frac{T\Delta}{2}\left( \frac{1}{b} - \frac{1}{a} \right) \\
%     \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}', \bar{c}')&\geq \mathbb{P}_{\bar{r}', \bar{c}'}\left( \tilde{T}_0(T) \geq T - \frac{T}{2b} + \frac{T}{2a}    \right) \frac{T\Delta}{2}\left( \frac{1}{b} - \frac{1}{a}\right) 
% \end{align*}
% Then, applying the Bretagnolle-Huber inequality from Theorem \ref{lemma::bretagnole_huber}:
% \begin{align}
%      \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}, \bar{c}) + \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}', \bar{c}') &\geq \frac{T\Delta}{2b} \left(\mathbb{P}_{\bar{r}, \bar{c}}\left( \tilde{T}_0(T) \leq T - \frac{T}{2b}    \right) + \mathbb{P}_{\bar{r}', \bar{c}'}\left( \tilde{T}_0(T) \geq T - \frac{T}{2b}    \right) \right) \notag \\
%      &\geq \frac{T\Delta}{2b} \exp\left( - D(\mathbb{P}_{\bar{r}, \bar{c}} ,  \mathbb{P}_{\bar{r}', \bar{c}'}) \right) \label{equation::supporting_lower_bound_huber}.
% \end{align}
% It remains to upper bound $ D(\mathbb{P}_{\bar{r}, \bar{c}} ,  \mathbb{P}_{\bar{r}', \bar{c}'})$. For this we use Lemma \ref{lemma::divergence_decomposition} and Lemma \ref{lemma::gaussian_divergence}, along with the definitions of $(\bar{r}, \bar{c})$ and $(\bar{r}', \bar{c}')$ to get:
% \begin{align*}
%     D(\mathbb{P}_{\bar{r}, \bar{c}} ,  \mathbb{P}_{\bar{r}', \bar{c}'})  &= \mathbb{E}_{\bar{r}, \bar{c}}\left[  T_i(T)   \right] D\left(\mathcal{N}( \binom{0}{a\tau}, \mathbb{I}_2), \mathcal{N}(\binom{2\Delta}{b\tau}, \mathbb{I}_2)\right)\\
%     &\leq \frac{T}{a (K-1)} D\left(\mathcal{N}( \binom{0}{a\tau}, \mathbb{I}_2), \mathcal{N}(\binom{2\Delta}{b\tau}, \mathbb{I}_2)\right) \\
%     &\leq  \frac{ T (4\Delta^2 + (a-b)^2)}{2a (K-1)}
% \end{align*}
% The first inequality follows by Equation \ref{equation::upper_bound_T_i}, the second one by Lemma \ref{lemma::gaussian_divergence}. Plugging this result back into inequality \ref{equation::supporting_lower_bound_huber} yields:
% \begin{equation*}
%      \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}, \bar{c}) + \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}', \bar{c}') \geq \frac{T\Delta}{2b}\exp\left( -     \frac{ T (4\Delta^2 + (a-b)^2)}{2a (K-1)} \right).
% \end{equation*}

% \end{proof}

















% \begin{theorem}
% Let $K > 1 $ and $T \geq K-1$. Then, for any algorithm $\mathcal{A}$, there is a pair of mean vectors $\bar{r}, \bar{c} \in [0,1]^K$ such that (where $c_0 = 0$ and $\tau$):
% \begin{equation*}
%     \mathcal{R}_\Pi(T) \geq \frac{1}{27} \sqrt{ }
% \end{equation*}
% \end{theorem}

% \begin{proof}
% Fix algorithm $\mathcal{A}$. Let $\Delta \in [0,1/2], 1 \leq b \leq a \leq \frac{1}{\tau}$ be come constants that will be chosen later. We start with a constrained Gaussian bandit instance with unit variances and mean rewards $\bar{r} = (\Delta, 0, \cdots, 0)$ and costs $\bar{c} = (0, a\tau, \cdots, a\tau)$. This environment gives rise to the distribution $\mathbb{P}_{\nu_{\bar{r}, \bar{c}}, \mathcal{A}}$ in the cannonical bandit model. For brevity we will use $\mathbb{P}_{\bar{r}, \bar{c}}$ instead of $\mathbb{P}_{\nu_{\bar{r}, \bar{c}}, \mathcal{A}}$, and expectations under $\mathbb{P}_{\bar{r}, \bar{c}}$ will be denoted by $\mathbb{E}_{\bar{r}, \bar{c}}$. 

% Let's index the arms from $0$ to $K-1$. We assume arm $0$ is the safe arm with known cost $0$ and unknown mean reward $\Delta$. Let $\pi_1, \cdots, \pi_T$ be the policies proposed by $\mathcal{A}$ during the run of the algorithm. For any $i \in \{ 0, \cdots K-1\}$ let $\tilde{T}_i = \sum_{t=1}^T \pi_t(i)$ be the total mass allocated by $\mathcal{A}$ to action $i$. 

% Let $i = \arg\min_{j> 0} \mathbb{E}_{\bar{r}, \bar{c}} [ \tilde{T}_j(T)]$. Notice that any feasibile policy $\pi_t$ satisfies $\pi_t(j) \leq \frac{1}{a}$, and therefore since $\sum_{j=1}^K \tilde{T}_j(T) = T$:
% \begin{equation*}
%     \mathbb{E}_{\bar{r}, \bar{c}}[ \tilde{T}_i(T)  ] \leq \frac{T}{a(K-1) } 
% \end{equation*}
% Furthermore, since for all $j\in \{0, \cdots, K-1\}$ it follows that $\mathbb{E}_{\bar{r}, \bar{c}}[T_j(T)] =  \mathbb{E}_{\bar{r}, \bar{c}}[\tilde{T}_j(T)] $, we conclude that:
% \begin{equation}\label{equation::upper_bound_T_i}
%     \mathbb{E}_{\bar{r}, \bar{c}}[ T_i(T)  ] \leq \frac{T}{a(K-1) } 
% \end{equation}
% Let's build a second constrained  Gaussian bandit instance with unit variances and mean rewards $\bar{r}' = (\Delta, 0, \cdots, 2\Delta, 0,\cdots, 0)$ and costs $\bar{c}'= (0, a\tau, \cdots, b\tau, \cdots, a\tau)$ where specifically $\bar{r}'_i = 2\Delta$ and $\bar{c}'_i = b\tau$. Therefore $\bar{r}_j = \bar{r}_j'$ and $\bar{c}_j  = \bar{c}_j'$ except at index $i$. Let $\mathbb{P}_{\bar{r}', \bar{c}'}$ be the distribution induced by environment $\bar{r}', \bar{c}'$. The optimal policy $\pi^{*}$ for $\mathbb{P}_{\bar{r}, \bar{c}}$ is to deterministically play the safe action $0$, the optimal policy $\underline{\pi}^{*}$ for $\mathbb{P}_{\bar{r}', \bar{c}'}$ is to play the mixture policy that selects arm $0$ with probability $1-\frac{1}{b}$ and arm $i$ with probability $\frac{1}{b}$. Policy $\pi^*$ has value $\Delta$ in $\mathbb{P}_{\bar{r}, \bar{c}}$ and policy $\underline{\pi}^{*}$ has value $\Delta + \frac{\Delta}{b}$ in $\mathbb{P}_{\bar{r}', \bar{c}'}$. A simple calculation leads to:
% \begin{align*}
%     \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}, \bar{c})&\geq \mathbb{P}_{\bar{r}, \bar{c}}\left( \tilde{T}_0(T) \leq T - \frac{T}{2b}    \right) \frac{T\Delta}{2b} \\
%     \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}', \bar{c}')&\geq \mathbb{P}_{\bar{r}', \bar{c}'}\left( \tilde{T}_0(T) \geq T - \frac{T}{2b}    \right) \frac{T\Delta}{2b} 
% \end{align*}
% Then, applying the Bretagnolle-Huber inequality from Theorem \ref{lemma::bretagnole_huber}:
% \begin{align}
%      \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}, \bar{c}) + \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}', \bar{c}') &\geq \frac{T\Delta}{2b} \left(\mathbb{P}_{\bar{r}, \bar{c}}\left( \tilde{T}_0(T) \leq T - \frac{T}{2b}    \right) + \mathbb{P}_{\bar{r}', \bar{c}'}\left( \tilde{T}_0(T) \geq T - \frac{T}{2b}    \right) \right) \notag \\
%      &\geq \frac{T\Delta}{2b} \exp\left( - D(\mathbb{P}_{\bar{r}, \bar{c}} ,  \mathbb{P}_{\bar{r}', \bar{c}'}) \right) \label{equation::supporting_lower_bound_huber}.
% \end{align}
% It remains to upper bound $ D(\mathbb{P}_{\bar{r}, \bar{c}} ,  \mathbb{P}_{\bar{r}', \bar{c}'})$. For this we use Lemma \ref{lemma::divergence_decomposition} and Lemma \ref{lemma::gaussian_divergence}, along with the definitions of $(\bar{r}, \bar{c})$ and $(\bar{r}', \bar{c}')$ to get:
% \begin{align*}
%     D(\mathbb{P}_{\bar{r}, \bar{c}} ,  \mathbb{P}_{\bar{r}', \bar{c}'})  &= \mathbb{E}_{\bar{r}, \bar{c}}\left[  T_i(T)   \right] D\left(\mathcal{N}( \binom{0}{a\tau}, \mathbb{I}_2), \mathcal{N}(\binom{2\Delta}{b\tau}, \mathbb{I}_2)\right)\\
%     &\leq \frac{T}{a (K-1)} D\left(\mathcal{N}( \binom{0}{a\tau}, \mathbb{I}_2), \mathcal{N}(\binom{2\Delta}{b\tau}, \mathbb{I}_2)\right) \\
%     &\leq  \frac{ T (4\Delta^2 + \tau^2 (a-b)^2)}{2a (K-1)}
% \end{align*}
% The first inequality follows by Equation \ref{equation::upper_bound_T_i}, the second one by Lemma \ref{lemma::gaussian_divergence}. Plugging this result back into inequality \ref{equation::supporting_lower_bound_huber} yields:
% \begin{equation*}
%      \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}, \bar{c}) + \mathcal{R}_\Pi( T, \mathcal{A}, \bar{r}', \bar{c}') \geq \frac{T\Delta}{2b}\exp\left( -     \frac{ T (4\Delta^2 + \tau^2(a-b)^2)}{2a (K-1)} \right).
% \end{equation*}

% Let $a = b = 4$ and set $\tau(a-b) = 2\Delta$. 


% \end{proof}
% There is still a gap between our lower and upper bounds. We conjecture that a tighter analysis can ... 

==> Constrained Bandits/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Constrained Bandits/multi_armed_bandits.tex <==
\section{Constrained Multi-Armed Bandits}
\label{sec:constrained-MAB}

In this section, we specialize our results for contextual linear bandits to multi-armed bandits (MAB) and show that the structure of the MAB problem allows a computationally efficient implementation of the algorithm and an improvement in the regret bound.  

In the MAB setting, the action set consists of $K$ arms $\mathcal{A}=\{1,\ldots,K\}$. Each arm $a\in [K]$ has a reward and a cost distribution with means $\bar{r}_a,\bar{c}_a\in [0,1]$. In each round $t\in[T]$, the agent constructs a policy $\pi_t$ over $\mathcal A$, pulls an arm $a_t\sim\pi_t$, and observes a reward-cost pair $(r_{a_t},c_{a_t})$ sampled i.i.d.~from the reward and cost distributions of arm $a_t$. Similar to the constrained contextual linear case, the goal of the agent is to produce a sequence of policies $\{\pi_t\}_{t=1}^T$ with maximum expected cumulative reward over $T$ rounds, i.e.,~$\sum_{t=1}^T\mathbb E_{a_t\sim\pi_t}[\bar{r}_{a_t}]$, while satisfying the {\bf\em linear constraint} $\mathbb E_{a_t\sim\pi_t}[\bar{c}_{a_t}] \leq \tau,\;\forall t\in[T]$. Moreover, arm $1$ is assumed to be the known safe arm, i.e.,~$\bar{c}_1 \leq \tau$. 

{\bf Optimistic Pessimistic Bandit (OPB) Algorithm.} $\;$ Let $\{T_a(t)\}_{a=1}^K$ and $\{\widehat{r}_a(t),\widehat{c}_a(t)\}_{a=1}^K$ be the total number of times that arm $a$ has been pulled and the estimated mean reward and cost of arm $a$ up until round $t$. In each round $t\in[T]$, OPB relies on the high-probability upper-bounds on the mean reward and cost of the arms, i.e.,~$\{u_a^r(t),u_a^c(t)\}_{a=1}^K$, where $u_a^r(t) = \widehat{r}_a(t) + \alpha_r\beta_a(t)$, $u_a^c(t) = \widehat{c}_a(t) + \alpha_c\beta_a(t)$, $\beta_a(t) = \sqrt{2\log(1/\delta')/T_a(t)}$, and constants $\alpha_r,\alpha_c\geq 1$. In order to produce a feasible policy, OPB solves the following linear program (LP) in each round $t\in[T]$: 

\vspace{-0.125in}
\begin{small}
\begin{equation}
\label{eq::noisy_LP}
\max_{\pi\in\Delta_K} \; \sum_{a\in\mathcal{A}}\pi_a \; u^r_a(t), \qquad\quad \text{s.t.} \; \sum_{a\in\mathcal{A}}\pi_a \; u_a^c(t) \leq \tau.
\end{equation}
\end{small}
\vspace{-0.125in}

As shown in~\eqref{eq::noisy_LP}, OPB selects its policy by being optimistic about reward (using an upper-bound for $r$) and pessimistic about cost (using an upper-bound for $c$). We report the details of OPB and its pseudo-code (Algorithm~\ref{alg::optimism_pessimism}) in Appendix~\ref{section::appendix_MAB_optimism_pessimism_algorithm}.

% \paragraph{Optimism Pessimism} Because we are interested in producing a feasible policy at all times, our algorithms solve a Linear Program balancing optimism on its reward while being pessimistic about its cost. More precisely, at time $t$ we play the policy $\pi_t$ resulting from solving the following LP:
% %
% \begin{align*}
% \label{eq::noisy_LP}
% \tag{$\widehat{\text{P}}_t$} 
% &\max_{\pi\in\mathrm{\Delta}_K} \;\; \sum_{a \in \mathcal{A}} \pi_a \; u^r_a(t) \qquad\;\;\; \longleftarrow \mathrm{Optimism} \\
% &\;\text{s.t.} \quad\; \sum_{a \in \mathcal{A}} \pi_a \; u_a^c(t)\leq \tau, \quad \longleftarrow \mathrm{Pessimism}
% \end{align*}

{\bf Computational Complexity of OPB.} $\;$ Unlike OPLB, whose optimization problem might be complex, OPB can be implemented extremely efficiently. Lemma~\ref{lemma::LP_support}, whose proof we report in Appendix~\ref{section::LP_structure_appendix}, show that~\eqref{eq::noisy_LP} always has a solution (policy) with support of at most $2$. This property allows us to solve~\eqref{eq::noisy_LP} in closed form, without a LP solver, and implement OPB quite efficiently. 

\begin{lemma}%[$\pi^*$ support]
\label{lemma::LP_support} 
There exists a policy that solves~\eqref{eq::noisy_LP} and has at most $2$ non-zero entries.
%The optimization problem~\eqref{} re exists an optimal solution of (\ref{eq::no_noise_LP}) with at most $2$ non-zero entries. 
\end{lemma}

%The proof is in Appendix~\ref{section::LP_structure_appendix}.

{\bf Regret Analysis of OPB.} $\;$ We prove the following regret-bound for OPB in Appendix~\ref{section:regret_analysis_appendix}. 

\begin{theorem}[Regret of OPB]
\label{theorem::contrained_MAB}
Let $\delta = 4KT\delta'$, $\alpha_c=1$, and $\alpha_r = 1+2/(\tau-\bar{c}_1)$. Then, with probability at least $1-\delta$, the regret of OPB satisfies

\vspace{-0.15in}
\begin{small}
\begin{equation*}
\mathcal{R}_\Pi(T) \leq \big(1 + \frac{2}{\tau-\bar{c}_1}\big) \times \big(2\sqrt{2KT\log(4KT/\delta)} + 4\sqrt{T\log(2/\delta)\log(4KT/\delta)}\big).
\end{equation*}
\end{small}
\vspace{-0.15in}
%
\end{theorem}

%The Extension of Theorem \ref{theorem::contrained_MAB} is straightforward and left to the appendix. 

The main component in the proof of Theorem~\ref{theorem::contrained_MAB} is the following lemma, whose proof is reported in Appendix~\ref{section:regret_analysis_appendix}. This lemma is the analogous to Lemma~\ref{lemma:linear_bandits_optimism} in the contextual linear bandit case. 

\begin{lemma}
\label{lemma::optimism}
If we set the parameters $\alpha_r$ and $\alpha_c$, such that $\alpha_r,\alpha_c\geq 1$ and $\alpha_c \leq (\tau-\bar{c}_1)(\alpha_r-1)$, then with high probability, for any $t\in[T]$, we have $\mathbb{E}_{a \sim \pi_t}\left[u_a^r(t)\right] \geq \mathbb{E}_{a \sim \pi^*}\left[\bar{r}_a \right]$.
\end{lemma}

Our contextual linear bandit formulation is general enough to include MAB. The regret analysis of OPLB (Theorem~\ref{theorem::main_theorem_linear}) yields a regret bound of order $\widetilde{\mathcal O}(\frac{K\sqrt{T}}{\tau-\bar{c}_1})$ for MAB. However, our OPB regret bound in Theorem~\ref{theorem::contrained_MAB} is of order $\widetilde{\mathcal O}(\frac{\sqrt{KT}}{\tau-\bar{c}_1})$, which shows a $\sqrt{K}$ improvement over simply casting MAB as an instance of contextual linear bandit and using the regret bound of OPLB. %as stated in Theorem~\ref{theorem::main_theorem_linear}. 

%\mgh{TODO ALDO: Write a few lines about the fact that we can easily extend things to $m$ constraints.} 

{\bf Extension to $m$ Constraints.} $\;$ In this case, the agent receives $m$ cost signals after pulling each arm. The cost vector of the safe arm $\boldsymbol{c}_1$ satisfies $\boldsymbol{c}_1(i)<\tau_i,\forall i\in[m]$, where $\{\tau_i\}_{i=1}^m$ are the constraint thresholds. Similar to single-constraint OPB, multi-constraint OPB is also computationally efficient. The main reason is that the LP of $m$-constraint OPB has a solution with at most $m+1$ non-zero entries. We obtain a regret bound of $\widetilde{\mathcal{O}}(\frac{\sqrt{KT }}{ \min_i \tau_i - \boldsymbol{c}_1(i)})$ for $m$-constraint OPB in Appendix~\ref{section::multiple_constraints_appendix}.

% We generalize these guarantees to the multiple constraints case in Appendix \ref{section::multiple_constraints_appendix}. In this setup the learner receives $M$ cost signals when pulling an arm, and it is required to play policies satisfying an expected cost constraints $\{ \tau_i\}_{i=1}^m$ on all cost signals at once. The learner has access to a safe arm with known cost values $\{c_1^{(i)}\}_{i=1}^M$ satisfying $c_1^{(i)} < \tau_i$ for all $i = 1, \cdots, m$. OPB extends naturally and tractably to the multiple constraint setting. In Appendix~\ref{section::multiple_constraints_appendix} we obtain a regret guarantee for the multiple constraints problem of the form $\tilde{\mathcal{O}}(\frac{\sqrt{KT }}{ \min \tau_i - c_1^{(i)}})$. Our proof uses the fact that to ensure the optimism argument in Lemma~\ref{lemma::optimism} to go through, it is enough to ensure $\frac{\alpha_r}{\alpha_c}\approx \frac{1}{ \min \tau_i - c_1^{(i)}}$, the inverse minimum gap. In this Lemma 5 becomes ... things are active. 


%\mgh{Some intuition for this would be good.}

{\bf Lower-bound.} $\;$ We also prove a mini-max lower-bound for this constrained MAB problem that shows no algorithm can attain a regret better than $\mathcal{O}(\max(\sqrt{KT}, \frac{1}{(\tau - \bar{c}_1)^2} ) )$. The formal statement of the lower-bound and the proof are reported in Appendix~\ref{section::lower_bound_MAB_appendix}.

==> Constrained Bandits/previous_work.tex <==
\section{Related Work}
\label{sec:related-work}
\vspace{-0.1in}

As described in Section~\ref{sec:intro}, our setting is the closest to the one studied by~\cite{amani2019linear} and~\cite{Moradipari19SL}. They study a slightly different setting, in which the mean cost of the action that the agent takes should satisfy the constraint, i.e.,~$\langle x_t,\mu_*\rangle \leq \tau$, not the mean cost of the policy it computes, i.e.,~$\langle x_{\pi_t},\mu_*\rangle \leq \tau$, as in our case. Clearly, the setting studied in our paper is more relaxed, and thus, is expected to obtain more rewards.~\cite{Moradipari19SL} propose a TS algorithm for their setting and prove an $\widetilde{O}(d^{3/2}\sqrt{T}/\tau)$ regret bound for it. They restrict themselves to linear bandits, i.e.,~$\mathcal A_t=\mathcal A,\forall t\in[T]$, and the safe action being the origin, i.e.,~$x_0=\mathbf{0}$ and $c_0=0$. This is why $c_0$ does not appear in their bounds. They consider their action set to be any convex compact subset of $\mathbb R^d$ that contains the origin. Although later in their proofs, to guarantee that their algorithm does not violate the constraint in the first round, they require the action set to also contain the ball with radius $\tau/S$ around the origin. Therefore, our action set is more general than theirs. Moreover, unlike us, their action set does not allows their results to be immediately applicable to MAB. Our regret bound also has a better dependence on $d$ and $\log T$ than theirs, similar to the best regret results for UCB vs.~TS. However, their algorithm is TS, and thus, is less complex than ours. Although it can be still intractable, even when $\mathcal A$ is convex. They needed to do several approximations in order to make their algorithm tractable in their experiments. 

%In \cite{Moradipari19SL}, the authors study an slightly different formulation of the contextual linear bandit problem with linear constraints. They restrict themselves to the case where $x_0 =0$ (and therefore $c_0 = 0$) and $\mathcal{A}_t = \mathcal{A}$ for all $t$ and for some convex set $\mathcal{A}$. Their algorithm, Safe Linear Thompson Sampling, achieves a regret bound of order $\mathcal{O}(\frac{d^{3/2}\sqrt{T}}{\tau})$ which as they note is optimal in its $T-$dependence, but suffers from the same suboptimality in its dependence on $d$ as other Linear Thompson sampling approaches (see \cite{}). The authors do not talk about their bound's dependence on $\tau$.  Their algorithm proceeds in similar fashion to ours, 1) compute a set of safe actions $\mathcal{S}_t$, an 2) select which action to select by maximizing a linear function $\mathcal{S}_t$. Although step 2) could be computationally tractable if the safe set admits a representation that amicable to linear optimization, computing $\mathcal{S}_t$ could prove intractable, even when $\mathcal{A}_t$ is convex. In their experimental evaluation the authors of \cite{Moradipari19SL} make use of several approximates to make their algorithms tractable. Their algorithm and setup is not immediately applicable to the Multi Armed Bandit problem.

In~\cite{amani2019linear}, reward and cost have the same unknown parameter $\theta_*$, and the cost is defined as $c_t=x_t^\top B\theta_*\leq\tau$, where $B$ is a known matrix. They derive and analyze an explore-exploit algorithm for this setting. Although our rate is better than theirs, i.e.,~$\widetilde{O}(T^{2/3})$, our algorithm cannot immediately give a $\widetilde{O}(\sqrt{T})$ regret for their setting, unless in special cases. 

%Another related work \cite{amani2019linear} proposes a similar but non-identical setting.  Specifically in \cite{amani2019linear}, the cost constraint involves the same unknown parameter vector $\theta_*$ and takes the form $x^\top B \theta_* \leq \tau$, for some known matrix $B$. As such, no cost information is needed. While in our setting we try to ensure the expected cost of a policy is no larger than $\tau$, the objective in \cite{amani2019linear} is to play actions that individually satisfy the cost constraint. Despite our algorithm being unable to give us a regret guarantee scaling with $\sqrt{T}$ for their setting, it does so in some special cases. For example, when all $\mathcal{A}_t$ are convex and $B = I$, our results already improve on the order $T^{2/3}$ regret bound for their explore and commit algorithm.  




%\mgh{TODO}

% Multi-armed bandits \cite{langford2008epoch,audibert2010best,kleinberg2008multi} have had tremendous impact in machine learning with applications spanning wireless networks \cite{maghsudi2016multi}, sensors \cite{washburn2008application}, strategy games \cite{ontanon2013combinatorial}, and online marketing \cite{burtini2015improving}.

% Perhaps the most related work to ours is the conservative bandit \cite{wu2016conservative}, where the goal is to "model the challenge faced by a company wishing to explore new strategies to maximize revenue whilst simultaneously maintaining their revenue above a fixed baseline, uniformly over time". Our work also has the goal to maintain a constraint uniformly over time. In other words, the conservative bandit is precisely the special case of constrained bandits where the constraint is on the reward itself (rather than based on a general emitted side information with each pull).
% The conservative bandit has also been extended to the case of contextual linear bandits
%  \cite{kazerouni2017conservative}, while still maintain constraints on the reward itself. Extending our work in a similar fashion to contextual bandits is a future research direction.
 
%  Work on learning with constraints has recently been done in reinforcement learning where one learns the policy with convex constraints using no-regret learning algorithms to solve a zero-sum game \cite{miryoosefi2019reinforcement}. Our work focuses on maintaining general constraints uniformly over time with algorithms which uses a different so-called optimism-pessimism type strategy rather than the classical no-regret two-player game dynamics. Similar approaches to \cite{miryoosefi2019reinforcement} include \cite{agrawal2015contextual,balakrishnan2018using} in the contextual bandits setting.

% Bandits with knapsacks \cite{badanidiyuru2013bandits} also deals with learning under resource constraints and the algorithms presented in \cite{badanidiyuru2013bandits} involve solving the well-known knapsack dynamic programming problem. Bandits with knapsacks have also been extended to the case of contextual bandits \cite{agrawal2016linear} and the case of concave rewards and convex knapsacks \cite{agrawal2014bandits}. Our work can also be seen as learning under similar resource constraints, however our guarantees are made uniformly across time and under uncertainty and thus the knapsack solution is unable to solve our bandit problem.

% \cite{mannor2006online} studies the problem of online learning with constraints where the goal is to maximize the long-term reward subject to average constraints are satisfied along the sample path. They show that the best in-hindsight solution is not attainable but one in the convex hull is attainable. Our work focuses on satisfying constraints uniformly across time. 

% \cite{badanidiyuru2014resourceful} study the problem of resourceful contextual bandits where in the contextual bandit setting, the bandits also consume resources and is required to maintain the constraints through time and is designed for the contextual setting. Our work on the other hand focuses on the simple non-contextual setting and also tries to maintain constraints across time, but with uncertainty in the constraints. \cite{wu2015algorithms} also studies the problem of contextual bandits under constraints.

% if y
% Very recently, \cite{amani2019linear} proposed linear bandits under safety constraints where the safety constraints are in the form of linear constraints that need to be satisfied at each time step.

\section{Conclusions}
\label{sec:conclu}
\vspace{-0.1in}

We derived a UCB-style algorithm for a new constrained contextual linear bandit setting, in which the goal is to produce a sequence of policies with maximum expected cumulative reward, while each policy has an expected cost below a certain threshold $\tau$. We proved a $T$-round regret bound of $\widetilde{\mathcal{O}}(\frac{d\sqrt{T}}{\tau-c_0})$ for our algorithm, which shows that the difficulty of the problem depends on the difference between the constraint threshold and the cost of a known feasible action $c_0$. We further specialized our results to MAB and proposed and analyzed a computationally efficient algorithm for this setting. We also proved a lower-bound for our constrained bandit problem and provided simulations to validate our theoretical results. A future direction is to use the optimism-pessimism idea behind our algorithm in other constrained bandit settings, including deriving a UCB-style algorithm for the setting studied in~\cite{amani2019linear} and~\cite{Moradipari19SL}. 

%\mgh{The mention of lower-bound should be removed here, in case we do not have it.}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

